Exact solutions of the relativistic Boltzmann equation in the relaxation time approximation

This Thesis concentrates on the analysis of coupled RTA (relaxation time approximation) kinetic equations for bosons and fermions. Bosons are treated as massless particles, while fermions have a finite mass. Using analytic and numerical methods we find exact solutions for such a mixture in the case of one-dimensional, boost-invariant expansion (for systems which are transversally homogeneous). In this way, several earlier results obtained for one-component systems and classical particles are generalized.

==> hydro_review.tex <==

@article{Mrowczynski:2005ki,
      author         = "Mrowczynski, Stanislaw",
      title          = "{Instabilities driven equilibration of the quark-gluon
                        plasma}",
      journal        = "Acta Phys. Polon.",
      volume         = "B37",
      year           = "2006",
      pages          = "427-454",
      eprint         = "hep-ph/0511052",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0511052;%%"
}

@article{vanderSchee:2013pia,
      author         = "van der Schee, Wilke and Romatschke, Paul and Pratt,
                        Scott",
      title          = "{Fully Dynamical Simulation of Central Nuclear
                        Collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "111",
      year           = "2013",
      number         = "22",
      pages          = "222302",
      doi            = "10.1103/PhysRevLett.111.222302",
      eprint         = "1307.2539",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1307.2539;%%"
}


@article{Berges:2013eia,
      author         = "Berges, Juergen and Boguslavski, Kirill and Schlichting, Soeren and
                        Venugopalan, Raju",
      title          = "{Turbulent thermalization process in heavy-ion collisions
                        at ultrarelativistic energies}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "7",
      pages          = "074011",
      doi            = "10.1103/PhysRevD.89.074011",
      eprint         = "1303.5650",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1303.5650;%%"
}


@article{Casher:1978wy,
      author         = "Casher, Aharon and Neuberger, Herbert and Nussinov, Shmuel~N.",
      title          = "{Chromoelectric Flux Tube Model of Particle Production}",
      journal        = "Phys. Rev.",
      volume         = "D20",
      year           = "1979",
      pages          = "179-188",
      doi            = "10.1103/PhysRevD.20.179",
      reportNumber   = "TAUP-694-78",
      SLACcitation   = "%%CITATION = PHRVA,D20,179;%%"
}

@article{Ryblewski:2013eja,
      author         = "Ryblewski, Radoslaw and Florkowski, Wojciech",
      title          = "{Equilibration of anisotropic quark-gluon plasma produced
                        by decays of color flux tubes}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      pages          = "034028",
      doi            = "10.1103/PhysRevD.88.034028",
      eprint         = "1307.0356",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1307.0356;%%"
}

@article{PRESSCUT-2000-210,
      title         = "{New State of Matter created at CERN. Un nouvel état de
                       la matière}",
      number        = "PRESSCUT-2000-210. CERN-PR-2000-01-EN. CERN-PR-2000-01-FR",
      pages         = "mult. p",
      year          = "2000",
      reportNumber  = "PRESSCUT-2000-210",
      url           = "https://cds.cern.ch/record/716634",
      note          = "Issued on 10 Feb 2000",
}


@article{Broniowski:2001we,
      author         = "Broniowski, Wojciech and Florkowski, Wojciech",
      title          = "{Explanation of the RHIC p(T) spectra in a thermal model
                        with expansion}",
      journal        = "Phys. Rev. Lett.",
      volume         = "87",
      year           = "2001",
      pages          = "272302",
      doi            = "10.1103/PhysRevLett.87.272302",
      eprint         = "nucl-th/0106050",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0106050;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%% recent books and reviews

@article{Alqahtani:2017mhy,
      author         = "Alqahtani, Mubarak and Nopoush, Mohammad and Strickland,
                        Michael",
      title          = "{Relativistic anisotropic hydrodynamics}",
      journal        = "Prog. Part. Nucl. Phys.",
      volume         = "101",
      year           = "2018",
      pages          = "204-248",
      doi            = "10.1016/j.ppnp.2018.05.004",
      eprint         = "1712.03282",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1712.03282;%%"
}
@article{Romatschke:2017ejr,
      author         = "Romatschke, Paul and Romatschke, Ulrike",
      title          = "{Relativistic Fluid Dynamics In and Out of Equilibrium --
                        Ten Years of Progress in Theory and Numerical Simulations
                        of Nuclear Collisions}",
      year           = "2017",
      eprint         = "1712.05815",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1712.05815;%%"
}
@book{Bartke2008,
author = {Bartke, Jerzy},
title = {Introduction to Relativistic Heavy Ion Physics},
publisher = {WORLD SCIENTIFIC},
year = {2008},
doi = {10.1142/1881},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/1881},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/1881}
}
@book{letessier_rafelski_2002, place={Cambridge}, series={Cambridge Monographs on Particle Physics, Nuclear Physics and Cosmology}, title={Hadrons and Quark–Gluon Plasma}, DOI={10.1017/CBO9780511534997}, publisher={Cambridge University Press}, author={Letessier, Jean and Rafelski, Johann}, year={2002}, collection={Cambridge Monographs on Particle Physics, Nuclear Physics and Cosmology}}

@book{Wong1994,
author = {Wong, Cheuk-Yin},
title = {Introduction to High-Energy Heavy-Ion Collisions},
publisher = {WORLD SCIENTIFIC},
year = {1994},
doi = {10.1142/1128},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/1128},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/1128}
}

@book{Hwa1990,
author = {Hwa, Rudolph C.},
title = {Quark-Gluon Plasma},
publisher = {WORLD SCIENTIFIC},
year = {1990},
doi = {10.1142/0498},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/0498},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/0498}
}
@book{Hwa2004,
author = {Hwa, Rudolph C. and Wang, Xin-Nian},
title = {Quark–Gluon Plasma 3},
publisher = {WORLD SCIENTIFIC},
year = {2004},
doi = {10.1142/5029},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/5029},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/5029}
}
@book{Wang2016,
author = {Wang, Xin-Nian},
title = {Quark–Gluon Plasma 5},
publisher = {WORLD SCIENTIFIC},
year = {2016},
doi = {10.1142/9533},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/9533},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/9533}
}

@book{Hwa1995,
author = {Hwa, Rudolph C.},
title = {Quark-Gluon Plasma 2},
publisher = {WORLD SCIENTIFIC},
year = {1995},
doi = {10.1142/2878},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/2878},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/2878}
}

@book{Hwa2010,
author = {Hwa, Rudolph C. and Wang, Xin-Nian},
title = {Quark-Gluon Plasma 4},
publisher = {WORLD SCIENTIFIC},
year = {2010},
doi = {10.1142/7588},
address = {},
edition   = {},
URL = {https://www.worldscientific.com/doi/abs/10.1142/7588},
eprint = {https://www.worldscientific.com/doi/pdf/10.1142/7588}
}

@book{LLfluid,
    author = {Landau, Lev D. and Lifshitz, Evgenij M.},
    title = {Fluid Mechanics, Second Edition: Volume 6 (Course of Theoretical Physics)},
    year = {1987}
}

@book{rezzolla2013relativistic,
  title={Relativistic Hydrodynamics},
  author={Rezzolla, Luciano and Zanotti, Olindo},
  year={2013},
  publisher={OUP Oxford}
}


@article{Heller:2016gbp,
      author         = "Heller, Michal P.",
      title          = "{Holography, Hydrodynamization and Heavy-Ion Collisions}",
      booktitle      = "{Proceedings, 56th Cracow School of Theoretical Physics :
                        A Panorama of Holography: Zakopane, Poland, May 24-June 1,
                        2016}",
      journal        = "Acta Phys. Polon.",
      volume         = "B47",
      year           = "2016",
      pages          = "2581",
      doi            = "10.5506/APhysPolB.47.2581",
      eprint         = "1610.02023",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1610.02023;%%"
}




@article{CasalderreySolana:2011us,
      author         = "Casalderrey-Solana, Jorge and Liu, Hong and Mateos, David
                        and Rajagopal, Krishna and Wiedemann, Urs Achim",
      title          = "{Gauge/String Duality, Hot QCD and Heavy Ion Collisions}",
      year           = "2011",
      doi            = "10.1017/CBO9781139136747",
      eprint         = "1101.0618",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CERN-PH-TH-2010-316, MIT-CTP-4198, ICCUB-10-202",
      SLACcitation   = "%%CITATION = ARXIV:1101.0618;%%"
}

@article{DeWolfe:2013cua,
      author         = "DeWolfe, Oliver and Gubser, Steven S. and Rosen,
                        Christopher and Teaney, Derek",
      title          = "{Heavy ions and string theory}",
      journal        = "Prog. Part. Nucl. Phys.",
      volume         = "75",
      year           = "2014",
      pages          = "86-132",
      doi            = "10.1016/j.ppnp.2013.11.001",
      eprint         = "1304.7794",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "COLO-HEP-579, PUPT-2446, CCTP-2013-06",
      SLACcitation   = "%%CITATION = ARXIV:1304.7794;%%"
}

@article{Kostadt:2000ty,
      author         = "Kostadt, Peter and Liu, Mario",
      title          = "{Causality and stability of the relativistic diffusion
                        equation}",
      journal        = "Phys. Rev.",
      volume         = "D62",
      year           = "2000",
      pages          = "023003",
      doi            = "10.1103/PhysRevD.62.023003",
      SLACcitation   = "%%CITATION = PHRVA,D62,023003;%%"
}

@article{Baier:2006um,
      author         = "Baier, Rudolf and Romatschke, Paul and Wiedemann, Urs
                        Achim",
      title          = "{Dissipative hydrodynamics and heavy ion collisions}",
      journal        = "Phys. Rev.",
      volume         = "C73",
      year           = "2006",
      pages          = "064903",
      doi            = "10.1103/PhysRevC.73.064903",
      eprint         = "hep-ph/0602249",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BI-TP-2006-04, RBRC-589",
      SLACcitation   = "%%CITATION = HEP-PH/0602249;%%"
}


@article{Romatschke:2009kr,
      author         = "Romatschke, Paul",
      title          = "{Relativistic Viscous Fluid Dynamics and Non-Equilibrium
                        Entropy}",
      journal        = "Class. Quant. Grav.",
      volume         = "27",
      year           = "2010",
      pages          = "025006",
      doi            = "10.1088/0264-9381/27/2/025006",
      eprint         = "0906.4787",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "INT-PUB-09-032",
      SLACcitation   = "%%CITATION = ARXIV:0906.4787;%%"
}

@article{Romatschke:2009im,
      author         = "Romatschke, Paul",
      title          = "{New Developments in Relativistic Viscous Hydrodynamics}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "E19",
      year           = "2010",
      pages          = "1-53",
      doi            = "10.1142/S0218301310014613",
      eprint         = "0902.3663",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "INT-PUB-09-010",
      SLACcitation   = "%%CITATION = ARXIV:0902.3663;%%"
}

@article{Jeon:2015dfa,
      author         = "Jeon, Sangyong and Heinz, Ulrich",
      title          = "{Introduction to Hydrodynamics}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "E24",
      year           = "2015",
      number         = "10",
      pages          = "1530010",
      doi            = "10.1142/S0218301315300106",
      eprint         = "1503.03931",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1503.03931;%%"
}

@article{Yagi:2005yb,
      author         = "Yagi, Kohsuke and Hatsuda, Tetsuo and Miake, Yasuo",
      title          = "{Quark-gluon plasma: From big bang to little bang}",
      journal        = "Camb. Monogr. Part. Phys. Nucl. Phys. Cosmol.",
      volume         = "23",
      year           = "2005",
      pages          = "1-446",
      SLACcitation   = "%%CITATION = CMPCE,23,1;%%"
}

@book{Vogt:2007zz,
      author         = "Vogt, Ramona",
      title          = "{Ultrarelativistic heavy-ion collisions}",
      publisher      = "Elsevier",
      address        = "Amsterdam",
      year           = "2007",
      ISBN           = "978-0-444-52196-5",
      SLACcitation   = "%%CITATION = INSPIRE-767840;%%"
}

@book{Florkowski:2010zz,
      author         = "Florkowski, Wojciech",
      title          = "{Phenomenology of Ultra-Relativistic Heavy-Ion
                        Collisions}",
      journal        = "Singapore, Singapore: World Scientific (2010) 416 p",
      year           = "2010",
      reportNumber   = "ISBN-9789814280662",
      SLACcitation   = "%%CITATION = ISBN-9789814280662;%%"
}

@article{Petreczky:2012rq,
      author         = "Petreczky, P.",
      title          = "{Lattice QCD at non-zero temperature}",
      journal        = "J. Phys.",
      volume         = "G39",
      year           = "2012",
      pages          = "093002",
      doi            = "10.1088/0954-3899/39/9/093002",
      eprint         = "1203.5320",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = ARXIV:1203.5320;%%"
}

@article{Ollitrault:2012cm,
      author         = "Ollitrault, Jean-Yves and Gardim, Fernando G.",
      title          = "{Hydro overview}",
      booktitle      = "{Proceedings, 23rd International Conference on
                        Ultrarelativistic Nucleus-Nucleus Collisions : Quark
                        Matter 2012 (QM 2012): Washington, DC, USA, August 13-18,
                        2012}",
      journal        = "Nucl. Phys.",
      volume         = "A904-905",
      year           = "2013",
      pages          = "75c-82c",
      doi            = "10.1016/j.nuclphysa.2013.01.047",
      eprint         = "1210.8345",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "SACLAY-T12-104",
      SLACcitation   = "%%CITATION = ARXIV:1210.8345;%%"
}


@article{Gale:2013da,
      author         = "Gale, Charles and Jeon, Sangyong and Schenke, Bjoern",
      title          = "{Hydrodynamic Modeling of Heavy-Ion Collisions}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "A28",
      year           = "2013",
      pages          = "1340011",
      doi            = "10.1142/S0217751X13400113",
      eprint         = "1301.5893",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1301.5893;%%"
}


@article{Florkowski:2017olj,
      author         = "Florkowski, Wojciech and Heller, Michal P. and Spalinski,
                        Michal",
      title          = "{New theories of relativistic hydrodynamics in the LHC
                        era}",
      journal        = "Rept. Prog. Phys.",
      volume         = "81",
      year           = "2018",
      number         = "4",
      pages          = "046001",
      doi            = "10.1088/1361-6633/aaa091",
      eprint         = "1707.02282",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1707.02282;%%"
}


@article{Stoecker:1986ci,
      author         = "Stoecker, Horst and Greiner, W.",
      title          = "{High-Energy Heavy Ion Collisions: Probing the Equation
                        of State of Highly Excited Hadronic Matter}",
      journal        = "Phys. Rept.",
      volume         = "137",
      year           = "1986",
      pages          = "277-392",
      doi            = "10.1016/0370-1573(86)90131-6",
      SLACcitation   = "%%CITATION = PRPLC,137,277;%%"
}

@article{Muller:1994rb,
      author         = "Muller, Berndt",
      title          = "{Physics and signatures of the quark-gluon plasma}",
      journal        = "Rept. Prog. Phys.",
      volume         = "58",
      year           = "1995",
      pages          = "611-636",
      doi            = "10.1088/0034-4885/58/6/002",
      eprint         = "nucl-th/9410005",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "DUKE-TH-94-76",
      SLACcitation   = "%%CITATION = NUCL-TH/9410005;%%"
}


@book{Csernai:1994xw,
      author         = "Csernai, L. P.",
      title          = "{Introduction to relativistic heavy ion collisions}",
      journal        = "Chichester, UK: Wiley (1994) 310 p",
      year           = "1994",
      SLACcitation   = "%%CITATION = INSPIRE-376250;%%"
}


@article{Mrowczynski:1998jr,
      author         = "Mrowczynski, Stanislaw",
      title          = "{Quark - gluon plasma}",
      booktitle      = "{New quantum phases, elementary excitations and
                        renormalization in high-energy, and condensed matter
                        physics. Proceedings, 38th Cracow School of Theoretical
                        Physics, Zakopane, Poland, June 1-10, 1998}",
      journal        = "Acta Phys. Polon.",
      volume         = "B29",
      year           = "1998",
      pages          = "3711",
      eprint         = "nucl-th/9905005",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/9905005;%%"
}


@book{Chaudhuri:2012yt,
      author         = "Chaudhuri, Asis~K.",
      title          = "{A short course on Relativistic Heavy Ion Collisions}",
      publisher      = "IOPP",
      year           = "2014",
      doi            = "10.1088/978-0-750-31060-4",
      eprint         = "1207.7028",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      ISBN           = "9780750310611, 9780750310604",
      SLACcitation   = "%%CITATION = ARXIV:1207.7028;%%"
}

@article{Satz:2018oiz,
      author         = "Satz, Helmut",
      title          = "{Extreme States of Matter in Strong Interaction Physics}",
      journal        = "Lect. Notes Phys.",
      volume         = "945",
      year           = "2018",
      pages          = "pp.1-288",
      doi            = "10.1007/978-3-319-71894-1",
      SLACcitation   = "%%CITATION = LNPHA,945,pp.1;%%"
}

@inproceedings{Bhalerao:2014owa,
      author         = "Bhalerao, Rajeev S.",
      title          = "{Relativistic heavy-ion collisions}",
      booktitle      = "{Proceedings, 1st Asia-Europe-Pacific School of
                        High-Energy Physics (AEPSHEP): Fukuoka, Japan, October
                        14-27, 2012}",
      year           = "2014",
      pages          = "219-239",
      doi            = "10.5170/CERN-2014-001.219",
      eprint         = "1404.3294",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "TIFR-TH-14-11",
      SLACcitation   = "%%CITATION = ARXIV:1404.3294;%%"
}


@article{Busza:2018rrf,
      author         = "Busza, Wit and Rajagopal, Krishna and van der Schee,
                        Wilke",
      title          = "{Heavy Ion Collisions: The Big Picture, and the Big
                        Questions}",
      year           = "2018",
      eprint         = "1802.04801",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIT-CTP-4892",
      SLACcitation   = "%%CITATION = ARXIV:1802.04801;%%"
}

@article{Yan:2017ivm,
      author         = "Yan, Li",
      title          = "{A flow paradigm in heavy-ion collisions}",
      journal        = "Chin. Phys.",
      volume         = "C42",
      year           = "2018",
      number         = "4",
      pages          = "042001",
      doi            = "10.1088/1674-1137/42/4/042001",
      eprint         = "1712.04580",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1712.04580;%%"
}

@article{Shuryak:1978ij,
      author         = "Shuryak, Edward V.",
      title          = "{Quark-Gluon Plasma and Hadronic Production of Leptons,
                        Photons and Psions}",
      journal        = "Phys. Lett.",
      volume         = "78B",
      year           = "1978",
      pages          = "150",
      doi            = "10.1016/0370-2693(78)90370-2",
      note           = "[Yad. Fiz.28,796(1978)]",
      reportNumber   = "IYF-78-24",
      SLACcitation   = "%%CITATION = PHLTA,78B,150;%%"
}

@article{Shuryak:1980tp,
      author         = "Shuryak, Edward V.",
      title          = "{Quantum Chromodynamics and the Theory of Superdense
                        Matter}",
      journal        = "Phys. Rept.",
      volume         = "61",
      year           = "1980",
      pages          = "71-158",
      doi            = "10.1016/0370-1573(80)90105-2",
      SLACcitation   = "%%CITATION = PRPLC,61,71;%%"
}


@article{Rafelski:1982pu,
      author         = "Rafelski, Johann and Muller, Berndt",
      title          = "{Strangeness Production in the Quark - Gluon Plasma}",
      journal        = "Phys. Rev. Lett.",
      volume         = "48",
      year           = "1982",
      pages          = "1066",
      doi            = "10.1103/PhysRevLett.48.1066, 10.1103/PhysRevLett.56.2334",
      note           = "[Erratum: Phys. Rev. Lett.56,2334(1986)]",
      reportNumber   = "Print-82-0048 (FRANKFURT)",
      SLACcitation   = "%%CITATION = PRLTA,48,1066;%%"
}

@article{Matsui:1986dk,
      author         = "Matsui, Tetsuo and Satz, Helmut",
      title          = "{$J/\psi$ Suppression by Quark-Gluon Plasma Formation}",
      journal        = "Phys. Lett.",
      volume         = "B178",
      year           = "1986",
      pages          = "416-422",
      doi            = "10.1016/0370-2693(86)91404-8",
      reportNumber   = "BNL-38344",
      SLACcitation   = "%%CITATION = PHLTA,B178,416;%%"
}
@inproceedings{Ryblewski:2017sgj,
      author         = "Ryblewski, Radoslaw",
      title          = "{Monte-Carlo statistical hadronization in relativistic
                        heavy-ion collisions}",
      booktitle      = "{53rd Winter School of Theoretical Physics: Understanding
                        the Origin of Matter from QCD Karpacz, Poland, February
                        26-March 4, 2017}",
      year           = "2017",
      eprint         = "1712.05213",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1712.05213;%%"
}

@inproceedings{Florkowski:2017ixx,
      author         = "Florkowski, Wojciech",
      title          = "{Hydrodynamic description of ultrarelativistic heavy-ion
                        collisions}",
      booktitle      = "{53rd Winter School of Theoretical Physics: Understanding
                        the Origin of Matter from QCD Karpacz, Poland, February
                        26-March 4, 2017}",
      year           = "2017",
      eprint         = "1712.05162",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1712.05162;%%"
}

@article{Florkowski:2017jnz,
      author         = "Florkowski, Wojciech and Maksymiuk, Ewa and Ryblewski,
                        Radoslaw",
      title          = "{Coupled kinetic equations for fermions and bosons in the
                        relaxation-time approximation}",
      journal        = "Phys. Rev.",
      volume         = "C97",
      year           = "2018",
      number         = "2",
      pages          = "024915",
      doi            = "10.1103/PhysRevC.97.024915",
      eprint         = "1710.07095",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1710.07095;%%"
}

@article{Florkowski:2017ovw,
      author         = "Florkowski, Wojciech and Maksymiuk, Ewa and Ryblewski,
                        Radoslaw",
      title          = "{Anisotropic-hydrodynamics approach to a quark-gluon
                        fluid mixture}",
      journal        = "Phys. Rev.",
      volume         = "C97",
      year           = "2018",
      number         = "1",
      pages          = "014904",
      doi            = "10.1103/PhysRevC.97.014904",
      eprint         = "1711.03872",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1711.03872;%%"
}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% other approaches to high order hydro

@article{Lublinsky:2007mm,
      author         = "Lublinsky, Michael and Shuryak, Edward",
      title          = "{How much entropy is produced in strongly coupled
                        Quark-Gluon Plasma (sQGP) by dissipative effects?}",
      journal        = "Phys. Rev.",
      volume         = "C76",
      year           = "2007",
      pages          = "021901",
      doi            = "10.1103/PhysRevC.76.021901",
      eprint         = "0704.1647",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0704.1647;%%"
}

@article{Lublinsky:2009kv,
      author         = "Lublinsky, Michael and Shuryak, Edward",
      title          = "{Improved Hydrodynamics from the AdS/CFT}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "065026",
      doi            = "10.1103/PhysRevD.80.065026",
      eprint         = "0905.4069",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0905.4069;%%"
}

@article{Bu:2014sia,
      author         = "Bu, Yanyan and Lublinsky, Michael",
      title          = "{All order linearized hydrodynamics from fluid-gravity
                        correspondence}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "8",
      pages          = "086003",
      doi            = "10.1103/PhysRevD.90.086003",
      eprint         = "1406.7222",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1406.7222;%%"
}

@article{Bu:2014ena,
      author         = "Bu, Yanyan and Lublinsky, Michael",
      title          = "{Linearized fluid/gravity correspondence: from shear
                        viscosity to all order hydrodynamics}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2014",
      pages          = "064",
      doi            = "10.1007/JHEP11(2014)064",
      eprint         = "1409.3095",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1409.3095;%%"
}

@article{Bu:2015bwa,
      author         = "Bu, Yanyan and Lublinsky, Michael and Sharon, Amir",
      title          = "{Hydrodynamics dual to Einstein-Gauss-Bonnet gravity:
                        all-order gradient resummation}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2015",
      pages          = "162",
      doi            = "10.1007/JHEP06(2015)162",
      eprint         = "1504.01370",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1504.01370;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%   CGC

@article{Lappi:2006fp,
      author         = "Lappi, Tuomas and McLerran, Larry~D.",
      title          = "{Some features of the glasma}",
      journal        = "Nucl. Phys.",
      volume         = "A772",
      year           = "2006",
      pages          = "200-212",
      doi            = "10.1016/j.nuclphysa.2006.04.001",
      eprint         = "hep-ph/0602189",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BNL-NT-06-10",
      SLACcitation   = "%%CITATION = HEP-PH/0602189;%%"
}


@article{McLerran:1993ni,
      author         = "McLerran, Larry~D. and Venugopalan, Raju",
      title          = "{Computing quark and gluon distribution functions for
                        very large nuclei}",
      journal        = "Phys. Rev.",
      volume         = "D49",
      year           = "1994",
      pages          = "2233-2241",
      doi            = "10.1103/PhysRevD.49.2233",
      eprint         = "hep-ph/9309289",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TPI-MINN-93-44-T, NUC-MINN-93-24-T, HEP-UMN-TH-1220-93",
      SLACcitation   = "%%CITATION = HEP-PH/9309289;%%"
}

@article{McLerran:1993ka,
      author         = "McLerran, Larry~D. and Venugopalan, Raju",
      title          = "{Gluon distribution functions for very large nuclei at
                        small transverse momentum}",
      journal        = "Phys. Rev.",
      volume         = "D49",
      year           = "1994",
      pages          = "3352-3355",
      doi            = "10.1103/PhysRevD.49.3352",
      eprint         = "hep-ph/9311205",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TPI-MINN-93-52-T, NUC-MINN-93-28-T, UMN-TH-1224-93",
      SLACcitation   = "%%CITATION = HEP-PH/9311205;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Glauber

@article{Bialas:1976ed,
      author         = "Bialas, Andrzej and Bleszynski, Marek and Czyz, Wieslaw",
      title          = "{Multiplicity Distributions in Nucleus-Nucleus Collisions
                        at High-Energies}",
      journal        = "Nucl. Phys.",
      volume         = "B111",
      year           = "1976",
      pages          = "461-476",
      doi            = "10.1016/0550-3213(76)90329-1",
      reportNumber   = "TPJU-9/76",
      SLACcitation   = "%%CITATION = NUPHA,B111,461;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    hydro calculations for RHIC

@article{Huovinen:2001cy,
      author         = "Huovinen, Pasi and Kolb, P. F. and Heinz, Ulrich W. and
                        Ruuskanen, Pentti~V. and Voloshin, S. A.",
      title          = "{Radial and elliptic flow at RHIC: Further predictions}",
      journal        = "Phys. Lett.",
      volume         = "B503",
      year           = "2001",
      pages          = "58-64",
      doi            = "10.1016/S0370-2693(01)00219-2",
      eprint         = "hep-ph/0101136",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0101136;%%"
}

@article{Teaney:2001av,
      author         = "Teaney, D. and Lauret, J. and Shuryak, E. V.",
      title          = "{A Hydrodynamic description of heavy ion collisions at
                        the SPS and RHIC}",
      year           = "2001",
      eprint         = "nucl-th/0110037",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0110037;%%"
}

@article{Kolb:2002ve,
      author         = "Kolb, Peter F. and Rapp, Ralf",
      title          = "{Transverse flow and hadrochemistry in Au+Au collisions
                        at $\sqrt{s_{\rm NN}}$ = 200~GeV}",
      journal        = "Phys. Rev.",
      volume         = "C67",
      year           = "2003",
      pages          = "044903",
      doi            = "10.1103/PhysRevC.67.044903",
      eprint         = "hep-ph/0210222",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SUNY-NTG-02-31",
      SLACcitation   = "%%CITATION = HEP-PH/0210222;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% AMY and related stuff

@article{Jeon:1995zm,
      author         = "Jeon, Sangyong and Yaffe, Laurence G.",
      title          = "{From quantum field theory to hydrodynamics: Transport
                        coefficients and effective kinetic theory}",
      journal        = "Phys. Rev.",
      volume         = "D53",
      year           = "1996",
      pages          = "5799-5809",
      doi            = "10.1103/PhysRevD.53.5799",
      eprint         = "hep-ph/9512263",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-95-09",
      SLACcitation   = "%%CITATION = HEP-PH/9512263;%%"
}

@article{Sasaki:2008fg,
      author         = "Sasaki, Chihiro and Redlich, Krzysztof",
      title          = "{Bulk viscosity in quasi particle models}",
      journal        = "Phys. Rev.",
      volume         = "C79",
      year           = "2009",
      pages          = "055207",
      doi            = "10.1103/PhysRevC.79.055207",
      eprint         = "0806.4745",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0806.4745;%%"
}

@article{Florkowski:2015rua,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and Su, Nan
                        and Tywoniuk, Konrad",
      title          = "{Bulk viscosity in a plasma of Gribov-Zwanziger gluons}",
      journal        = "Acta Phys. Polon.",
      volume         = "B47",
      year           = "2016",
      pages          = "1833",
      doi            = "10.5506/APhysPolB.47.1833",
      eprint         = "1504.03176",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ICCUB-15-014",
      SLACcitation   = "%%CITATION = ARXIV:1504.03176;%%"
}

@article{Florkowski:2015dmm,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and Su, Nan
                        and Tywoniuk, Konrad",
      title          = "{Transport coefficients of the Gribov-Zwanziger plasma}",
      journal        = "Phys. Rev.",
      volume         = "C94",
      year           = "2016",
      number         = "4",
      pages          = "044904",
      doi            = "10.1103/PhysRevC.94.044904",
      eprint         = "1509.01242",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1509.01242;%%"
}



@article{Baier:2000sb,
      author         = "Baier, Rudolf and Mueller, Alfred H. and Schiff, Dominique and Son,
                        Dam T.",
      title          = "{'Bottom up' thermalization in heavy ion collisions}",
      journal        = "Phys. Lett.",
      volume         = "B502",
      year           = "2001",
      pages          = "51-58",
      doi            = "10.1016/S0370-2693(01)00191-5",
      eprint         = "hep-ph/0009237",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0009237;%%"
}

@article{Arnold:2000dr,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Transport coefficients in high temperature gauge
                        theories. 1. Leading log results}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2000",
      pages          = "001",
      doi            = "10.1088/1126-6708/2000/11/001",
      eprint         = "hep-ph/0010177",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-00-15",
      SLACcitation   = "%%CITATION = HEP-PH/0010177;%%"
}

@article{Arnold:2001ba,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Photon emission from ultrarelativistic plasmas}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2001",
      pages          = "057",
      doi            = "10.1088/1126-6708/2001/11/057",
      eprint         = "hep-ph/0109064",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-01-21",
      SLACcitation   = "%%CITATION = HEP-PH/0109064;%%"
}

@article{Arnold:2001ms,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Photon emission from quark gluon plasma: Complete
                        leading order results}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2001",
      pages          = "009",
      doi            = "10.1088/1126-6708/2001/12/009",
      eprint         = "hep-ph/0111107",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-01-22",
      SLACcitation   = "%%CITATION = HEP-PH/0111107;%%"
}

@article{Arnold:2002ja,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Photon and gluon emission in relativistic plasmas}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2002",
      pages          = "030",
      doi            = "10.1088/1126-6708/2002/06/030",
      eprint         = "hep-ph/0204343",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-02-06",
      SLACcitation   = "%%CITATION = HEP-PH/0204343;%%"
}

@article{Arnold:2002zm,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Effective kinetic theory for high temperature gauge
                        theories}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2003",
      pages          = "030",
      doi            = "10.1088/1126-6708/2003/01/030",
      eprint         = "hep-ph/0209353",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0209353;%%"
}

@article{Arnold:2003zc,
      author         = "Arnold, Peter Brockway and Moore, Guy D and Yaffe,
                        Laurence G.",
      title          = "{Transport coefficients in high temperature gauge
                        theories. 2. Beyond leading log}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2003",
      pages          = "051",
      doi            = "10.1088/1126-6708/2003/05/051",
      eprint         = "hep-ph/0302165",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0302165;%%"
}

@article{Arnold:2004ti,
      author         = "Arnold, Peter Brockway and Lenaghan, Jonathan and Moore,
                        Guy D. and Yaffe, Laurence G.",
      title          = "{Apparent thermalization due to plasma instabilities in
                        quark-gluon plasma}",
      journal        = "Phys. Rev. Lett.",
      volume         = "94",
      year           = "2005",
      pages          = "072302",
      doi            = "10.1103/PhysRevLett.94.072302",
      eprint         = "nucl-th/0409068",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0409068;%%"
}

@article{Arnold:2005vb,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{The Fate of non-Abelian plasma instabilities in 3+1
                        dimensions}",
      journal        = "Phys. Rev.",
      volume         = "D72",
      year           = "2005",
      pages          = "054003",
      doi            = "10.1103/PhysRevD.72.054003",
      eprint         = "hep-ph/0505212",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0505212;%%"
}

@article{Arnold:2014jva,
      author         = "Arnold, Peter and Romatschke, Paul and van der Schee,
                        Wilke",
      title          = "{Absence of a local rest frame in far from equilibrium
                        quantum matter}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2014",
      pages          = "110",
      doi            = "10.1007/JHEP10(2014)110",
      eprint         = "1408.2518",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1408.2518;%%"
}

@article{Arnold:1997gh,
      author         = "Arnold, Peter Brockway and Yaffe, Laurence G.",
      title          = "{Effective theories for real time correlations in hot
                        plasmas}",
      journal        = "Phys. Rev.",
      volume         = "D57",
      year           = "1998",
      pages          = "1178-1192",
      doi            = "10.1103/PhysRevD.57.1178",
      eprint         = "hep-ph/9709449",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UW-PT-97-22",
      SLACcitation   = "%%CITATION = HEP-PH/9709449;%%"
}

@article{Hartnoll:2005ju,
      author         = "Hartnoll, Sean A. and Kumar, S. Prem",
      title          = "{AdS black holes and thermal Yang-Mills correlators}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2005",
      pages          = "036",
      doi            = "10.1088/1126-6708/2005/12/036",
      eprint         = "hep-th/0508092",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DAMTP-2005-73",
      SLACcitation   = "%%CITATION = HEP-TH/0508092;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Kurkela EKT

@article{Kurkela:2014tea,
      author         = "Kurkela, Aleksi and Lu, Egang",
      title          = "{Approach to Equilibrium in Weakly Coupled Non-Abelian
                        Plasmas}",
      journal        = "Phys. Rev. Lett.",
      volume         = "113",
      year           = "2014",
      number         = "18",
      pages          = "182301",
      doi            = "10.1103/PhysRevLett.113.182301",
      eprint         = "1405.6318",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2014-093",
      SLACcitation   = "%%CITATION = ARXIV:1405.6318;%%"
}

@article{Kurkela:2015qoa,
      author         = "Kurkela, Aleksi and Zhu, Yan",
      title          = "{Isotropization and hydrodynamization in weakly coupled
                        heavy-ion collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "115",
      year           = "2015",
      number         = "18",
      pages          = "182301",
      doi            = "10.1103/PhysRevLett.115.182301",
      eprint         = "1506.06647",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2015-142",
      SLACcitation   = "%%CITATION = ARXIV:1506.06647;%%"
}

@article{Keegan:2015avk,
      author         = "Keegan, Liam and Kurkela, Aleksi and Romatschke, Paul and
                        van der Schee, Wilke and Zhu, Yan",
      title          = "{Weak and strong coupling equilibration in nonabelian
                        gauge theories}",
      journal        = "JHEP",
      volume         = "04",
      year           = "2016",
      pages          = "031",
      doi            = "10.1007/JHEP04(2016)031",
      eprint         = "1512.05347",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CERN-PH-TH-2015-304, MIT-CTP-4750",
      SLACcitation   = "%%CITATION = ARXIV:1512.05347;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Czajka

@article{Czajka:2014gaa,
      author         = "Czajka, Alina and Mrowczynski, Stanislaw",
      title          = "{Universality of the hard-loop action}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "2",
      pages          = "025013",
      doi            = "10.1103/PhysRevD.91.025013",
      eprint         = "1410.5117",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1410.5117;%%"
}

@article{Czajka:2017bod,
      author         = "Czajka, Alina and Jeon, Sangyong",
      title          = "{Kubo formulas for the shear and bulk viscosity
                        relaxation times and the scalar field theory shear
                        $\tau_\pi$ calculation}",
      journal        = "Phys. Rev.",
      volume         = "C95",
      year           = "2017",
      number         = "6",
      pages          = "064906",
      doi            = "10.1103/PhysRevC.95.064906",
      eprint         = "1701.07580",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1701.07580;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%%%
%% VISCOSITY BOUND

@article{Danielewicz:1984ww,
      author         = "Danielewicz, Pawel and Gyulassy, Miklos",
      title          = "{Dissipative Phenomena in Quark Gluon Plasmas}",
      journal        = "Phys. Rev.",
      volume         = "D31",
      year           = "1985",
      pages          = "53-62",
      doi            = "10.1103/PhysRevD.31.53",
      SLACcitation   = "%%CITATION = PHRVA,D31,53;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%   gradient expansion


@article{Geroch:2001xs,
      author         = "Geroch, Robert P.",
      title          = "{On hyperbolic 'theories' of relativistic dissipative
                        fluids}",
      year           = "2001",
      eprint         = "gr-qc/0103112",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = GR-QC/0103112;%%"
}


@article{Hiscock:1985zz,
      author         = "Hiscock, William A. and Lindblom, Lee",
      title          = "{Generic instabilities in first-order dissipative
                        relativistic fluid theories}",
      journal        = "Phys.Rev.",
      volume         = "D31",
      pages          = "725-733",
      doi            = "10.1103/PhysRevD.31.725",
      year           = "1985",
      SLACcitation   = "%%CITATION = PHRVA,D31,725;%%",
}



@article{Denicol:2011fa,
      author         = "Denicol, Gabriel~S. and Noronha, Jorge and Niemi, Harri
                        and Rischke, Dirk~H.",
      title          = "{Origin of the Relaxation Time in Dissipative Fluid
                        Dynamics}",
      journal        = "Phys.Rev.",
      volume         = "D83",
      pages          = "074019",
      doi            = "10.1103/PhysRevD.83.074019",
      year           = "2011",
      eprint         = "1102.4780",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1102.4780;%%",
}

@article{Denicol:2012es,
      author         = "Denicol, Gabriel~S. and Molnar, Etele and Niemi, Harri and Rischke,
                        Dirk~H.",
      title          = "{Derivation of fluid dynamics from kinetic theory with
                        the 14--moment approximation}",
      journal        = "Eur. Phys. J. A",
      volume         = "48",
      pages          = "170",
      doi            = "10.1140/epja/i2012-12170-x",
      year           = "2012",
      eprint         = "1206.1554",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1206.1554;%%",
}


@article{Heller:2013fn,
      author         = "Heller, Michal P. and Janik, Romuald A. and Witaszczyk,
                        Przemyslaw",
      title          = "{Hydrodynamic Gradient Expansion in Gauge Theory
                        Plasmas}",
      journal        = "Phys.Rev.Lett.",
      number         = "21",
      volume         = "110",
      pages          = "211602",
      doi            = "10.1103/PhysRevLett.110.211602",
      year           = "2013",
      eprint         = "1302.0697",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1302.0697;%%",
}

@article{Heller:2015dha,
      author         = "Heller, Michal P. and Spalinski, Michal",
      title          = "{Hydrodynamics Beyond the Gradient Expansion: Resurgence
                        and Resummation}",
      journal        = "Phys. Rev. Lett.",
      volume         = "115",
      year           = "2015",
      number         = "7",
      pages          = "072501",
      doi            = "10.1103/PhysRevLett.115.072501",
      eprint         = "1503.07514",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1503.07514;%%"
}



@article{Aniceto:2015mto,
      author         = "Aniceto, Ines and Spalinski, Michal",
      title          = "{Resurgence in Extended Hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "8",
      pages          = "085008",
      doi            = "10.1103/PhysRevD.93.085008",
      eprint         = "1511.06358",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1511.06358;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%   collective degrees of freedom


@article{Baier:2007ix,
      author         = "Baier, Rudolf and Romatschke, Paul and Son, Dam Thanh and
                        Starinets, Andrei O. and Stephanov, Mikhail~A.",
      title          = "{Relativistic viscous hydrodynamics, conformal
                        invariance, and holography}",
      journal        = "JHEP",
      volume         = "04",
      year           = "2008",
      pages          = "100",
      doi            = "10.1088/1126-6708/2008/04/100",
      eprint         = "0712.2451",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "BI-TP-2007-29, INT-PUB-07-45, SHEP-07-47",
      SLACcitation   = "%%CITATION = ARXIV:0712.2451;%%"
}

@article{Bhattacharya:2011eea,
      author         = "Bhattacharya, Jyotirmoy and Bhattacharyya, Sayantani and
                        Minwalla, Shiraz",
      title          = "{Dissipative Superfluid dynamics from gravity}",
      journal        = "JHEP",
      volume         = "04",
      year           = "2011",
      pages          = "125",
      doi            = "10.1007/JHEP04(2011)125",
      eprint         = "1101.3332",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "TIFR-TH-11-15",
      SLACcitation   = "%%CITATION = ARXIV:1101.3332;%%"
}

@article{Heller:2014wfa,
      author         = "Heller, Michal P. and Janik, Romuald A. and Spalinski,
                        Michal and Witaszczyk, Przemyslaw",
      title          = "{Coupling hydrodynamics to nonequilibrium degrees of
                        freedom in strongly interacting quark-gluon plasma}",
      journal        = "Phys.Rev.Lett.",
      number         = "26",
      volume         = "113",
      pages          = "261601",
      doi            = "10.1103/PhysRevLett.113.261601",
      year           = "2014",
      eprint         = "1409.5087",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1409.5087;%%",
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RTA

@article{Bhatnagar:1954zz,
      author         = "Bhatnagar, Prabhu~L. and Gross, Eilam~P. and Krook, Max",
      title          = "{A Model for Collision Processes in Gases. 1. Small
                        Amplitude Processes in Charged and Neutral One-Component
                        Systems}",
      journal        = "Phys. Rev.",
      volume         = "94",
      year           = "1954",
      pages          = "511-525",
      doi            = "10.1103/PhysRev.94.511",
      SLACcitation   = "%%CITATION = PHRVA,94,511;%%"
}

@article{Heller:2016rtz,
      author         = "Heller, Michal P. and Kurkela, Aleksi and Spalinski,
                        Michal",
      title          = "{Hydrodynamization and transient modes of expanding
                        plasma in kinetic theory}",
      year           = "2016",
      eprint         = "1609.04803",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1609.04803;%%"
}

@article{Denicol:2016bjh,
      author         = "Denicol, Gabriel S. and Noronha, Jorge",
      title          = "{Divergence of the Chapman-Enskog expansion in
                        relativistic kinetic theory}",
      year           = "2016",
      eprint         = "1608.07869",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1608.07869;%%"
}

@article{Blaizot:2017lht,
      author         = "Blaizot, John~P. and Yan, Li",
      title          = "{Onset of hydrodynamics for a quark-gluon plasma from the
                        evolution of moments of distribution functions}",
      year           = "2017",
      eprint         = "1703.10694",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1703.10694;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MIS

@article{Muller:1967zza,
      author         = "Muller, Ingo",
      title          = "{Zum Paradoxon der Warmeleitungstheorie}",
      journal        = "Z. Phys.",
      volume         = "198",
      year           = "1967",
      pages          = "329-344",
      doi            = "10.1007/BF01326412",
      SLACcitation   = "%%CITATION = ZEPYA,198,329;%%"
}

@article{Israel:1976tn,
      author         = "Israel, Werner",
      title          = "{Nonstationary irreversible thermodynamics: A Causal
                        relativistic theory}",
      journal        = "Annals Phys.",
      volume         = "100",
      year           = "1976",
      pages          = "310-331",
      doi            = "10.1016/0003-4916(76)90064-6",
      SLACcitation   = "%%CITATION = APNYA,100,310;%%"
}

@article{Israel:1979wp,
      author         = "Israel, Werner and Stewart, John~M.",
      title          = "{Transient relativistic thermodynamics and kinetic
                        theory}",
      journal        = "Annals Phys.",
      volume         = "118",
      year           = "1979",
      pages          = "341-372",
      doi            = "10.1016/0003-4916(79)90130-1",
      SLACcitation   = "%%CITATION = APNYA,118,341;%%"
}

%%%% implementations

@article{Heinz:2005bw,
      author         = "Heinz, Ulrich W. and Song, Huichao and Chaudhuri, Asis~K.",
      title          = "{Dissipative hydrodynamics for viscous relativistic
                        fluids}",
      journal        = "Phys. Rev.",
      volume         = "C73",
      year           = "2006",
      pages          = "034904",
      doi            = "10.1103/PhysRevC.73.034904",
      eprint         = "nucl-th/0510014",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0510014;%%"
}


@article{Karpenko:2013wva,
      author         = "Karpenko, Iu. and Huovinen, Pasi and Bleicher, M.",
      title          = "{A 3+1 dimensional viscous hydrodynamic code for
                        relativistic heavy ion collisions}",
      journal        = "Comput. Phys. Commun.",
      volume         = "185",
      year           = "2014",
      pages          = "3016-3027",
      doi            = "10.1016/j.cpc.2014.07.010",
      eprint         = "1312.4160",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1312.4160;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bjorken flow

@article{Gorenstein:1977xv,
      author         = "Gorenstein, Mark I. and Sinyukov, {\relax Yu}. M. and
                        Zhdanov, V. I.",
      title          = "{On Scaling Solutions in the Hydrodynamical Theory of
                        Multiparticle Production}",
      journal        = "Phys. Lett.",
      volume         = "B71",
      year           = "1977",
      pages          = "199-202",
      doi            = "10.1016/0370-2693(77)90777-8",
      SLACcitation   = "%%CITATION = PHLTA,B71,199;%%"
}


@article{Bjorken:1982qr,
      author         = "Bjorken, James~D.",
      title          = "{Highly Relativistic Nucleus-Nucleus Collisions: The
                        Central Rapidity Region}",
      journal        = "Phys. Rev.",
      volume         = "D27",
      year           = "1983",
      pages          = "140-151",
      doi            = "10.1103/PhysRevD.27.140",
      reportNumber   = "FERMILAB-PUB-82-044-THY, FERMILAB-PUB-82-044-T",
      SLACcitation   = "%%CITATION = PHRVA,D27,140;%%"
}

@article{Baym:1984sr,
      author         = "Baym, Gordon and Friman, Bengt~L. and Blaizot, John~P. and Soyeur, Madeleine and Czyz, Wieslaw",
      title          = "{Hydrodynamics of Ultrarelativistic Heavy Ion
                        Collisions}",
      booktitle      = "{Nucl. Phys. A407 ( 1983) 541-570, In *Odenthal-altenberg
                        1983, Proceedings, Recent Progress In Many-body Theories*,
                        60-67}",
      journal        = "Nucl. Phys.",
      volume         = "A407",
      year           = "1983",
      pages          = "541-570",
      doi            = "10.1016/0375-9474(83)90666-8",
      SLACcitation   = "%%CITATION = NUPHA,A407,541;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  problems with causality

@article{Lindblom:1995gp,
      author         = "Lindblom, Lee",
      title          = "{The Relaxation effect in dissipative relativistic fluid
                        theories}",
      journal        = "Annals Phys.",
      volume         = "247",
      year           = "1996",
      pages          = "1",
      doi            = "10.1006/aphy.1996.0036",
      eprint         = "gr-qc/9508058",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = GR-QC/9508058;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% DNMR

@article{Denicol:2010xn,
      author         = "Denicol, Gabriel S. and Koide, T. and Rischke, Dirk~H.",
      title          = "{Dissipative relativistic fluid dynamics: a new way to
                        derive the equations of motion from kinetic theory}",
      journal        = "Phys. Rev. Lett.",
      volume         = "105",
      year           = "2010",
      pages          = "162501",
      doi            = "10.1103/PhysRevLett.105.162501",
      eprint         = "1004.5013",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1004.5013;%%"
}

@article{Denicol:2012cn,
      author         = "Denicol, Gabriel~S. and Niemi, Harri and Molnar, Etele and Rischke,
                        Dirk~H.",
      title          = "{Derivation of transient relativistic fluid dynamics from
                        the Boltzmann equation}",
      journal        = "Phys. Rev.",
      volume         = "D85",
      year           = "2012",
      pages          = "114047",
      doi            = "10.1103/PhysRevD.85.114047, 10.1103/PhysRevD.91.039902",
      note           = "[Erratum: Phys. Rev.D91,no.3,039902(2015)]",
      eprint         = "1202.4551",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1202.4551;%%"
}

@article{Denicol:2014loa,
      author         = "Denicol, G. S.",
      title          = "{Kinetic foundations of relativistic dissipative fluid
                        dynamics}",
      journal        = "J. Phys.",
      volume         = "G41",
      year           = "2014",
      number         = "12",
      pages          = "124004",
      doi            = "10.1088/0954-3899/41/12/124004",
      SLACcitation   = "%%CITATION = JPAGA,G41,124004;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CHAPMAN-ENSKOG

@article{Jaiswal:2013npa,
      author         = "Jaiswal, Amaresh",
      title          = "{Relativistic dissipative hydrodynamics from kinetic
                        theory with relaxation time approximation}",
      journal        = "Phys. Rev.",
      volume         = "C87",
      year           = "2013",
      number         = "5",
      pages          = "051901",
      doi            = "10.1103/PhysRevC.87.051901",
      eprint         = "1302.6311",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1302.6311;%%"
}

%%% Jaiswal's third order hydro

@article{Jaiswal:2013vta,
      author         = "Jaiswal, Amaresh",
      title          = "{Relativistic third-order dissipative fluid dynamics from
                        kinetic theory}",
      journal        = "Phys. Rev.",
      volume         = "C88",
      year           = "2013",
      pages          = "021903",
      doi            = "10.1103/PhysRevC.88.021903",
      eprint         = "1305.3480",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1305.3480;%%"
}


@article{Jaiswal:2014raa,
      author         = "Jaiswal, Amaresh",
      title          = "{Relaxation-time approximation and relativistic
                        third-order viscous hydrodynamics from kinetic theory}",
      booktitle      = "{Proceedings, 24th International Conference on
                        Ultra-Relativistic Nucleus-Nucleus Collisions (Quark
                        Matter 2014): Darmstadt, Germany, May 19-24, 2014}",
      journal        = "Nucl. Phys.",
      volume         = "A931",
      year           = "2014",
      pages          = "1205-1210",
      doi            = "10.1016/j.nuclphysa.2014.08.035",
      eprint         = "1407.0837",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1407.0837;%%"
}

@article{Chattopadhyay:2014lya,
      author         = "Chattopadhyay, Chandrodoy and Jaiswal, Amaresh and Pal,
                        Subrata and Ryblewski, Radoslaw",
      title          = "{Relativistic third-order viscous corrections to the
                        entropy four-current from kinetic theory}",
      journal        = "Phys. Rev.",
      volume         = "C91",
      year           = "2015",
      number         = "2",
      pages          = "024917",
      doi            = "10.1103/PhysRevC.91.024917",
      eprint         = "1411.2363",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1411.2363;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% BRSSS


@article{Schenke:2011bn,
      author         = "Schenke, Bjorn and Jeon, Sangyong and Gale, Charles",
      title          = "{Higher flow harmonics from (3+1)D event-by-event viscous
                        hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C85",
      year           = "2012",
      pages          = "024901",
      doi            = "10.1103/PhysRevC.85.024901",
      eprint         = "1109.6289",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1109.6289;%%"
}

@article{Romatschke:2011qp,
      author         = "Romatschke, Paul",
      title          = "{Relativistic (Lattice) Boltzmann Equation with Non-Ideal
                        Equation of State}",
      journal        = "Phys. Rev.",
      volume         = "D85",
      year           = "2012",
      pages          = "065012",
      doi            = "10.1103/PhysRevD.85.065012",
      eprint         = "1108.5561",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1108.5561;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%   PRE  anisotropic hydrodynamics


@article{Barz:1987pq,
      author         = "Barz, H. W. and Kampfer, Burkhard and Lukacs, B. and
                        Martinas, K. and Wolf, G.",
      title          = "{Deconfinement transition in anisotropic matter}",
      journal        = "Phys. Lett.",
      volume         = "B194",
      year           = "1987",
      pages          = "15-19",
      doi            = "10.1016/0370-2693(87)90761-1",
      reportNumber   = "KFKI-1987-14/A",
      SLACcitation   = "%%CITATION = PHLTA,B194,15;%%"
}

@article{Kampfer:1990qg,
      author         = "Kampfer, Burkhard and Lukacs, B. and Wolf, G. and Barz,
                        H. W.",
      title          = "{Description of the nuclear stopping process within anisotropic thermo hydrodynamics}",
      booktitle      = "{NATO ASI: International Advanced Courses on The Nuclear
                        Equation of State Peniscola, Spain, May 21-June 3, 1989}",
      journal        = "Phys. Lett.",
      volume         = "B240",
      year           = "1990",
      pages          = "297-300",
      doi            = "10.1016/0370-2693(90)91101-G",
      reportNumber   = "KFKI-1990-03/A",
      SLACcitation   = "%%CITATION = PHLTA,B240,297;%%"
}

@article{Noronha:2011fi,
      author         = "Noronha, Jorge and Denicol, Gabriel S.",
      title          = "{Transient Fluid Dynamics of the Quark-Gluon Plasma
                        According to AdS/CFT}",
      year           = "2011",
      eprint         = "1104.2415",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1104.2415;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%   anisotropic hydrodynamics

@article{Florkowski:2010cf,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw",
      title          = "{Highly-anisotropic and strongly-dissipative
                        hydrodynamics for early stages of relativistic heavy-ion
                        collisions}",
      journal        = "Phys. Rev.",
      volume         = "C83",
      year           = "2011",
      pages          = "034907",
      doi            = "10.1103/PhysRevC.83.034907",
      eprint         = "1007.0130",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1007.0130;%%"
}

@article{Martinez:2010sc,
      author         = "Martinez, Mauricio and Strickland, Michael",
      title          = "{Dissipative Dynamics of Highly Anisotropic Systems}",
      journal        = "Nucl. Phys.",
      volume         = "A848",
      year           = "2010",
      pages          = "183-197",
      doi            = "10.1016/j.nuclphysa.2010.08.011",
      eprint         = "1007.0889",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1007.0889;%%"
}
@article{Florkowski:2014bba,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and
                        Strickland, Michael and Tinti, Leonardo",
      title          = "{Leading-order anisotropic hydrodynamics for systems with
                        massive particles}",
      journal        = "Phys. Rev.",
      volume         = "C89",
      year           = "2014",
      number         = "5",
      pages          = "054909",
      doi            = "10.1103/PhysRevC.89.054909",
      eprint         = "1403.1223",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1403.1223;%%"
}
@article{Nopoush:2015yga,
      author         = "Nopoush, Mohammad and Strickland, Michael and Ryblewski,
                        Radoslaw and Bazow, Dennis and Heinz, Ulrich and Martinez,
                        Mauricio",
      title          = "{Leading-order anisotropic hydrodynamics for central
                        collisions}",
      journal        = "Phys. Rev.",
      volume         = "C92",
      year           = "2015",
      number         = "4",
      pages          = "044912",
      doi            = "10.1103/PhysRevC.92.044912",
      eprint         = "1506.05278",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1506.05278;%%"
}

@article{Heinz:2004pj,
      author         = "Heinz, Ulrich W.",
      title          = "{Thermalization at RHIC}",
      booktitle      = "{Proceedings, 9th Hadron Physics and 7th Relativistic
                        Aspects of Nuclear Physics (HADRON-RANP 2004): A Joint
                        Meeting on QCD and QGP: Rio de Janeiro, Brazil, March
                        28-April 3, 2004}",
      journal        = "AIP Conf. Proc.",
      volume         = "739",
      year           = "2005",
      pages          = "163-180",
      doi            = "10.1063/1.1843595",
      note           = "[,163(2004)]",
      eprint         = "nucl-th/0407067",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0407067;%%"
}

@article{Florkowski:2012as,
      author         = "Florkowski, Wojciech and Maj, Radoslaw and Ryblewski,
                        Radoslaw and Strickland, Michael",
      title          = "{Hydrodynamics of anisotropic quark and gluon fluids}",
      journal        = "Phys. Rev.",
      volume         = "C87",
      year           = "2013",
      number         = "3",
      pages          = "034914",
      doi            = "10.1103/PhysRevC.87.034914",
      eprint         = "1209.3671",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1209.3671;%%"
}

@article{Florkowski:2013uqa,
      author         = "Florkowski, Wojciech and Maj, Radoslaw",
      title          = "{Mixture of anisotropic fluids}",
      journal        = "Acta Phys. Polon.",
      volume         = "B44",
      year           = "2013",
      number         = "10",
      pages          = "2003-2017",
      doi            = "10.5506/APhysPolB.44.2003",
      eprint         = "1309.2786",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1309.2786;%%"
}

@article{Florkowski:2014txa,
      author         = "Florkowski, Wojciech and Madetko, Oskar",
      title          = "{Kinetic description of mixtures of anisotropic fluids}",
      journal        = "Acta Phys. Polon.",
      volume         = "B45",
      year           = "2014",
      number         = "5",
      pages          = "1103-1118",
      doi            = "10.5506/APhysPolB.45.1103",
      eprint         = "1402.2401",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1402.2401;%%"
}


@article{Florkowski:2015cba,
      author         = "Florkowski, Wojciech and Maksymiuk, Ewa and Ryblewski,
                        Radoslaw and Tinti, Leonardo",
      title          = "{Anisotropic hydrodynamics for a mixture of quark and
                        gluon fluids}",
      journal        = "Phys. Rev.",
      volume         = "C92",
      year           = "2015",
      number         = "5",
      pages          = "054912",
      doi            = "10.1103/PhysRevC.92.054912",
      eprint         = "1508.04534",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1508.04534;%%"
}


@article{Romatschke:2016hle,
      author         = "Romatschke, Paul",
      title          = "{Do nuclear collisions create a locally equilibrated
                        quark-gluon plasma?}",
      journal        = "Eur. Phys. J.",
      volume         = "C77",
      year           = "2017",
      number         = "1",
      pages          = "21",
      doi            = "10.1140/epjc/s10052-016-4567-x",
      eprint         = "1609.02820",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1609.02820;%%"
}

@article{Romatschke:2017acs,
      author         = "Romatschke, Paul",
      title          = "{Relativistic Hydrodynamic Attractors with Broken
                        Symmetries: Non-Conformal and Non-Homogeneous}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2017",
      pages          = "079",
      doi            = "10.1007/JHEP12(2017)079",
      eprint         = "1710.03234",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1710.03234;%%"
}

@article{Ryblewski:2013jsa,
      author         = "Ryblewski, Radoslaw",
      title          = "{Anisotropic hydrodynamics for ultra-relativistic
                        heavy-ion collisions}",
      journal        = "J. Phys.",
      volume         = "G40",
      year           = "2013",
      pages          = "093101",
      doi            = "10.1088/0954-3899/40/9/093101",
      SLACcitation   = "%%CITATION = JPAGA,G40,093101;%%"
}

@article{Ryblewski:2010ch,
      author         = "Ryblewski, Radoslaw and Florkowski, Wojciech",
      title          = "{Highly anisotropic hydrodynamics -- discussion of the
                        model assumptions and forms of the initial conditions}",
      journal        = "Acta Phys. Polon.",
      volume         = "B42",
      year           = "2011",
      pages          = "115-138",
      doi            = "10.5506/APhysPolB.42.115",
      eprint         = "1011.6213",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1011.6213;%%"
}
@article{Ryblewski:2011aq,
      author         = "Ryblewski, Radoslaw and Florkowski, Wojciech",
      title          = "{Highly-anisotropic and strongly-dissipative
                        hydrodynamics with transverse expansion}",
      journal        = "Eur. Phys. J.",
      volume         = "C71",
      year           = "2011",
      pages          = "1761",
      doi            = "10.1140/epjc/s10052-011-1761-8",
      eprint         = "1103.1260",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1103.1260;%%"
}
@article{Ryblewski:2010bs,
      author         = "Ryblewski, Radoslaw and Florkowski, Wojciech",
      title          = "{Non-boost-invariant motion of dissipative and highly
                        anisotropic fluid}",
      journal        = "J. Phys.",
      volume         = "G38",
      year           = "2011",
      pages          = "015104",
      doi            = "10.1088/0954-3899/38/1/015104",
      eprint         = "1007.4662",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1007.4662;%%"
}

@article{Ryblewski:2012rr,
      author         = "Ryblewski, Radoslaw and Florkowski, Wojciech",
      title          = "{Highly-anisotropic hydrodynamics in 3+1 space-time
                        dimensions}",
      journal        = "Phys. Rev.",
      volume         = "C85",
      year           = "2012",
      pages          = "064901",
      doi            = "10.1103/PhysRevC.85.064901",
      eprint         = "1204.2624",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1204.2624;%%"
}





@article{Bazow:2015cha,
      author         = "Bazow, Dennis and Heinz, Ulrich W. and Martinez,
                        Mauricio",
      title          = "{Nonconformal viscous anisotropic hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C91",
      year           = "2015",
      number         = "6",
      pages          = "064903",
      doi            = "10.1103/PhysRevC.91.064903",
      eprint         = "1503.07443",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1503.07443;%%"
}


@article{Strickland:2015utc,
      author         = "Strickland, Michael and Nopoush, Mohammad and Ryblewski,
                        Radoslaw",
      title          = "{Anisotropic hydrodynamics for conformal Gubser flow}",
      booktitle      = "{Proceedings, 25th International Conference on
                        Ultra-Relativistic Nucleus-Nucleus Collisions (Quark
                        Matter 2015): Kobe, Japan, September 27-October 3, 2015}",
      journal        = "Nucl. Phys.",
      volume         = "A956",
      year           = "2016",
      pages          = "268-271",
      doi            = "10.1016/j.nuclphysa.2016.02.014",
      eprint         = "1512.07334",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1512.07334;%%"
}



@article{Alqahtani:2015qja,
      author         = "Alqahtani, Mubarak and Nopoush, Mohammad and Strickland,
                        Michael",
      title          = "{Quasiparticle equation of state for anisotropic
                        hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C92",
      year           = "2015",
      number         = "5",
      pages          = "054910",
      doi            = "10.1103/PhysRevC.92.054910",
      eprint         = "1509.02913",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1509.02913;%%"
}







@article{Alqahtani:2016rth,
      author         = "Alqahtani, Mubarak and Nopoush, Mohammad and Strickland,
                        Michael",
      title          = "{Quasiparticle anisotropic hydrodynamics for central
                        collisions}",
      journal        = "Phys. Rev.",
      volume         = "C95",
      year           = "2017",
      number         = "3",
      pages          = "034906",
      doi            = "10.1103/PhysRevC.95.034906",
      eprint         = "1605.02101",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1605.02101;%%"
}





@article{Alqahtani:2017tnq,
      author         = "Alqahtani, Mubarak and Nopoush, Mohammad and Ryblewski,
                        Radoslaw and Strickland, Michael",
      title          = "{Anisotropic hydrodynamic modeling of 2.76 TeV Pb-Pb
                        collisions}",
      journal        = "Phys. Rev.",
      volume         = "C96",
      year           = "2017",
      number         = "4",
      pages          = "044910",
      doi            = "10.1103/PhysRevC.96.044910",
      eprint         = "1705.10191",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1705.10191;%%"
}




%%%%%%%%  RS form %%%%%%%%%%



@article{Romatschke:2003ms,
      author         = "Romatschke, Paul and Strickland, Michael",
      title          = "{Collective modes of an anisotropic quark gluon plasma}",
      journal        = "Phys. Rev.",
      volume         = "D68",
      year           = "2003",
      pages          = "036004",
      doi            = "10.1103/PhysRevD.68.036004",
      eprint         = "hep-ph/0304092",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TUW-03-09",
      SLACcitation   = "%%CITATION = HEP-PH/0304092;%%"
}

@article{Florkowski:2008ag,
      author         = "Florkowski, Wojciech",
      title          = "{Anisotropic fluid dynamics in the early stage of
                        relativistic heavy-ion collisions}",
      journal        = "Phys. Lett.",
      volume         = "B668",
      year           = "2008",
      pages          = "32-35",
      doi            = "10.1016/j.physletb.2008.07.101",
      eprint         = "0806.2268",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:0806.2268;%%"
}


@article{Martinez:2012tu,
      author         = "Martinez, Mauricio and Ryblewski, Radoslaw and
                        Strickland, Michael",
      title          = "{Boost-Invariant (2+1)-dimensional Anisotropic
                        Hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C85",
      year           = "2012",
      pages          = "064913",
      doi            = "10.1103/PhysRevC.85.064913",
      eprint         = "1204.1473",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "INT-PUB-12-014",
      SLACcitation   = "%%CITATION = ARXIV:1204.1473;%%"
}

@article{Bazow:2013ifa,
      author         = "Bazow, Dennis and Heinz, Ulrich W. and Strickland,
                        Michael",
      title          = "{Second-order (2+1)-dimensional anisotropic
                        hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C90",
      year           = "2014",
      number         = "5",
      pages          = "054910",
      doi            = "10.1103/PhysRevC.90.054910",
      eprint         = "1311.6720",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1311.6720;%%"
}

@article{Strickland:2014pga,
      author         = "Strickland, Michael",
      title          = "{Anisotropic Hydrodynamics: Three lectures}",
      booktitle      = "{54th Cracow School of Theoretical Physics: QCD meets
                        experiment: Zakopane, Poland, June 12-20, 2014}",
      journal        = "Acta Phys. Polon.",
      volume         = "B45",
      year           = "2014",
      number         = "12",
      pages          = "2355-2394",
      doi            = "10.5506/APhysPolB.45.2355",
      eprint         = "1410.5786",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1410.5786;%%"
}
















































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%% %%%%

@article{Nopoush:2014pfa,
      author         = "Nopoush, Mohammad and Ryblewski, Radoslaw and Strickland,
                        Michael",
      title          = "{Bulk viscous evolution within anisotropic
                        hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C90",
      year           = "2014",
      number         = "1",
      pages          = "014908",
      doi            = "10.1103/PhysRevC.90.014908",
      eprint         = "1405.1355",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1405.1355;%%"
}

@article{Tinti:2014yya,
      author         = "Tinti, Leonardo",
      title          = "{(3?+?1)-dimensional framework for leading-order
                        nonconformal anisotropic hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C92",
      year           = "2015",
      number         = "1",
      pages          = "014908",
      doi            = "10.1103/PhysRevC.92.014908",
      eprint         = "1411.7268",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1411.7268;%%"
}

@article{Nopoush:2014qba,
      author         = "Nopoush, Mohammad and Ryblewski, Radoslaw and Strickland,
                        Michael",
      title          = "{Anisotropic hydrodynamics for conformal Gubser flow}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "4",
      pages          = "045007",
      doi            = "10.1103/PhysRevD.91.045007",
      eprint         = "1410.6790",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1410.6790;%%"
}



@article{Tinti:2015xra,
      author         = "Tinti, Leonardo and Ryblewski, Radoslaw and Florkowski,
                        Wojciech and Strickland, Michael",
      title          = "{Testing different formulations of leading-order
                        anisotropic hydrodynamics}",
      journal        = "Nucl. Phys.",
      volume         = "A946",
      year           = "2016",
      pages          = "29-48",
      doi            = "10.1016/j.nuclphysa.2015.11.006",
      eprint         = "1505.06456",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1505.06456;%%"
}

@article{Tinti:2015xwa,
      author         = "Tinti, Leonardo",
      title          = "{Anisotropic matching principle for the hydrodynamics
                        expansion}",
      journal        = "Phys. Rev.",
      volume         = "C94",
      year           = "2016",
      number         = "4",
      pages          = "044902",
      doi            = "10.1103/PhysRevC.94.044902",
      eprint         = "1506.07164",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1506.07164;%%"
}

@article{Molnar:2016vvu,
      author         = "Molnar, Etele and Niemi, Harri and Rischke, Dirk~H.",
      title          = "{Derivation of anisotropic dissipative fluid dynamics
                        from the Boltzmann equation}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "11",
      pages          = "114025",
      doi            = "10.1103/PhysRevD.93.114025",
      eprint         = "1602.00573",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1602.00573;%%"
}

@article{Molnar:2016gwq,
      author         = "Molnar, Etele and Niemi, Harri and Rischke, Dirk~H.",
      title          = "{Closing the equations of motion of anisotropic fluid
                        dynamics by a judicious choice of a moment of the
                        Boltzmann equation}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "12",
      pages          = "125003",
      doi            = "10.1103/PhysRevD.94.125003",
      eprint         = "1606.09019",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1606.09019;%%"
}

@article{Martinez:2017ibh,
      author         = "Martinez, M. and McNelis, M. and Heinz, U.",
      title          = "{Anisotropic fluid dynamics for Gubser flow}",
      journal        = "Phys. Rev.",
      volume         = "C95",
      year           = "2017",
      number         = "5",
      pages          = "054907",
      doi            = "10.1103/PhysRevC.95.054907",
      eprint         = "1703.10955",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1703.10955;%%"
}


@article{Damodaran:2017ior,
      author         = "Damodaran, Mridula and Molnar, Denes and Barnafoldi,
                        Gergely Gabor and Berenyi, Daniel and Ferenc Nagy-Egri,
                        Mate",
      title          = "{Testing and improving shear viscous phase space
                        correction models}",
      year           = "2017",
      eprint         = "1707.00793",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1707.00793;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% non-boost-invariant perfect and viscous hydrodynamics

@article{Florkowski:1992yd,
      author         = "Florkowski, Wojciech and Friman, Bengt~L. and Baym,
                        Gordon and Ruuskanen, Pentti~V.",
      title          = "{Convective stability of hot matter in ultrarelativistic
                        heavy ion collisions}",
      journal        = "Nucl. Phys.",
      volume         = "A540",
      year           = "1992",
      pages          = "659-674",
      doi            = "10.1016/0375-9474(92)90179-N",
      reportNumber   = "GSI-92-02",
      SLACcitation   = "%%CITATION = NUPHA,A540,659;%%"
}

@article{Satarov:2006iw,
      author         = "Satarov, L. M. and Merdeev, A. V. and Mishustin, I. N.
                        and Stoecker, Horst",
      title          = "{Longitudinal fluid-dynamics for ultrarelativistic
                        heavy-ion collisions}",
      journal        = "Phys. Rev.",
      volume         = "C75",
      year           = "2007",
      pages          = "024903",
      doi            = "10.1103/PhysRevC.75.024903",
      eprint         = "hep-ph/0606074",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0606074;%%"
}

@article{Bozek:2007qt,
      author         = "Bozek, Piotr",
      title          = "{Viscous evolution of the rapidity distribution of matter
                        created in relativistic heavy-ion collisions}",
      journal        = "Phys. Rev.",
      volume         = "C77",
      year           = "2008",
      pages          = "034911",
      doi            = "10.1103/PhysRevC.77.034911",
      eprint         = "0712.3498",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:0712.3498;%%"
}

@article{Floerchinger:2015efa,
      author         = "Floerchinger, Stefan and Martinez, Mauricio",
      title          = "{Fluid dynamic propagation of initial baryon number
                        perturbations on a Bjorken flow background}",
      journal        = "Phys. Rev.",
      volume         = "C92",
      year           = "2015",
      number         = "6",
      pages          = "064906",
      doi            = "10.1103/PhysRevC.92.064906",
      eprint         = "1507.05569",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "CERN-PH-TH-2015-169",
      SLACcitation   = "%%CITATION = ARXIV:1507.05569;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% anisotropic hydrodynamics vs. viscous hydrodynamics

@article{Baym:1984np,
      author         = "Baym, Gordon",
      title          = "{Thermal equilibration in ultra relativistic heavy-ion collisions}",
      journal        = "Phys. Lett.",
      volume         = "B138",
      year           = "1984",
      pages          = "18-22",
      doi            = "10.1016/0370-2693(84)91863-X",
      SLACcitation   = "%%CITATION = PHLTA,B138,18;%%"
}

@article{Baym:1985tna,
      author         = "Baym, Gordon",
      title          = "{Entropy production and the evolution of ultra relativistic heavy-ion collisions }",
      booktitle      = "{QUARK MATTER '83. PROCEEDINGS, 3RD INTERNATIONAL
                        CONFERENCE ON ULTRARELATIVISTIC NUCLEUS NUCLEUS
                        COLLISIONS, UPTON, USA, SEPTEMBER 26-30, 1983}",
      journal        = "Nucl. Phys.",
      volume         = "A418",
      year           = "1984",
      pages          = "525C-537C",
      doi            = "10.1016/0375-9474(84)90573-6",
      SLACcitation   = "%%CITATION = NUPHA,A418,525C;%%"
}


@article{Florkowski:2013lza,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and
                        Strickland, Michael",
      title          = "{Anisotropic Hydrodynamics for Rapidly Expanding
                        Systems}",
      journal        = "Nucl. Phys.",
      volume         = "A916",
      year           = "2013",
      pages          = "249-259",
      doi            = "10.1016/j.nuclphysa.2013.08.004",
      eprint         = "1304.0665",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1304.0665;%%"
}

@article{Florkowski:2013lya,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and
                        Strickland, Michael",
      title          = "{Testing viscous and anisotropic hydrodynamics in an
                        exactly solvable case}",
      journal        = "Phys. Rev.",
      volume         = "C88",
      year           = "2013",
      pages          = "024903",
      doi            = "10.1103/PhysRevC.88.024903",
      eprint         = "1305.7234",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1305.7234;%%"
}



@article{Florkowski:2014sfa,
      author         = "Florkowski, Wojciech and Maksymiuk, Ewa and Ryblewski,
                        Radoslaw and Strickland, Michael",
      title          = "{Exact solution of the (0+1)-dimensional Boltzmann
                        equation for a massive gas}",
      journal        = "Phys. Rev.",
      volume         = "C89",
      year           = "2014",
      number         = "5",
      pages          = "054908",
      doi            = "10.1103/PhysRevC.89.054908",
      eprint         = "1402.7348",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1402.7348;%%"
}

@article{Florkowski:2014sda,
      author         = "Florkowski, Wojciech and Maksymiuk, Ewa",
      title          = "{Exact solution of the (0+1)-dimensional Boltzmann
                        equation for massive Bose-Einstein and Fermi-Dirac gases}",
      journal        = "J. Phys.",
      volume         = "G42",
      year           = "2015",
      number         = "4",
      pages          = "045106",
      doi            = "10.1088/0954-3899/42/4/045106",
      eprint         = "1411.3666",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1411.3666;%%"
}


@article{Denicol:2014tha,
      author         = "Denicol, Gabriel S. and Heinz, Ulrich W. and Martinez,
                        Mauricio and Noronha, Jorge and Strickland, Michael",
      title          = "{Studying the validity of relativistic hydrodynamics with
                        a new exact solution of the Boltzmann equation}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "12",
      pages          = "125026",
      doi            = "10.1103/PhysRevD.90.125026",
      eprint         = "1408.7048",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1408.7048;%%"
}

@article{Denicol:2014xca,
      author         = "Denicol, Gabriel S. and Heinz, Ulrich W. and Martinez,
                        Mauricio and Noronha, Jorge and Strickland, Michael",
      title          = "{New Exact Solution of the Relativistic Boltzmann
                        Equation and its Hydrodynamic Limit}",
      journal        = "Phys. Rev. Lett.",
      volume         = "113",
      year           = "2014",
      number         = "20",
      pages          = "202301",
      doi            = "10.1103/PhysRevLett.113.202301",
      eprint         = "1408.5646",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1408.5646;%%"
}
@article{Florkowski:2016kjj,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and
                        Strickland, Michael and Tinti, Leonardo",
      title          = "{Non-boost-invariant dissipative hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C94",
      year           = "2016",
      number         = "6",
      pages          = "064903",
      doi            = "10.1103/PhysRevC.94.064903",
      eprint         = "1609.06293",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1609.06293;%%"
}



@article{Noronha:2015jia,
      author         = "Noronha, Jorge and Denicol, Gabriel S.",
      title          = "{Perfect fluidity of a dissipative system: Analytical
                        solution for the Boltzmann equation in
                        $\mathrm{AdS}_{2}\otimes \mathrm{S}_{2}$}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "11",
      pages          = "114032",
      doi            = "10.1103/PhysRevD.92.114032",
      eprint         = "1502.05892",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1502.05892;%%"
}
@article{Florkowski:2012ax,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and
                        Strickland, Michael",
      title          = "{Chromoelectric oscillations in a dynamically evolving
                        anisotropic background}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "085023",
      doi            = "10.1103/PhysRevD.86.085023",
      eprint         = "1207.0344",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1207.0344;%%"
}


@article{Florkowski:2015lra,
      author         = "Florkowski, Wojciech and Jaiswal, Amaresh and Maksymiuk,
                        Ewa and Ryblewski, Radoslaw and Strickland, Michael",
      title          = "{Relativistic quantum transport coefficients for
                        second-order viscous hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C91",
      year           = "2015",
      pages          = "054907",
      doi            = "10.1103/PhysRevC.91.054907",
      eprint         = "1503.03226",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1503.03226;%%"
}


@article{Denicol:2014mca,
      author         = "Denicol, Gabriel S. and Florkowski, Wojciech and
                        Ryblewski, Radoslaw and Strickland, Michael",
      title          = "{Shear-bulk coupling in nonconformal hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C90",
      year           = "2014",
      number         = "4",
      pages          = "044905",
      doi            = "10.1103/PhysRevC.90.044905",
      eprint         = "1407.4767",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1407.4767;%%"
}


@article{Jaiswal:2014isa,
      author         = "Jaiswal, Amaresh and Ryblewski, Radoslaw and Strickland,
                        Michael",
      title          = "{Transport coefficients for bulk viscous evolution in the
                        relaxation time approximation}",
      journal        = "Phys. Rev.",
      volume         = "C90",
      year           = "2014",
      number         = "4",
      pages          = "044908",
      doi            = "10.1103/PhysRevC.90.044908",
      eprint         = "1407.7231",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1407.7231;%%"
}


@article{Bemfica:2017wps,
      author         = "Bemfica, Fabio S. and Disconzi, Marcelo M. and Noronha,
                        Jorge",
      title          = "{Causality and existence of solutions of relativistic
                        viscous fluid dynamics with gravity}",
      year           = "2017",
      eprint         = "1708.06255",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1708.06255;%%"
}


@article{Ryblewski:2015psh,
      author         = "Ryblewski, Radoslaw",
      title          = "{Thermalization of parton spectra in the colour-flux-tube
                        model}",
      journal        = "J. Phys.",
      volume         = "G43",
      year           = "2016",
      number         = "9",
      pages          = "095102",
      doi            = "10.1088/0954-3899/43/9/095102",
      eprint         = "1512.04117",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1512.04117;%%"
}



@article{Florkowski:2016zsi,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw and
                        Spaliński, Michał",
      title          = "{Gradient expansion for anisotropic hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "11",
      pages          = "114025",
      doi            = "10.1103/PhysRevD.94.114025",
      eprint         = "1608.07558",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1608.07558;%%"
}

@article{Bazow:2015zca,
      author         = "Bazow, Dennis and Martinez, Mauricio and Heinz, Ulrich
                        W.",
      title          = "{Transient oscillations in a macroscopic effective theory
                        of the Boltzmann equation}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "3",
      pages          = "034002",
      doi            = "10.1103/PhysRevD.93.034002",
      note           = "[Phys. Rev.D93,034002(2016)]",
      eprint         = "1507.06595",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1507.06595;%%"
}

@article{HellerSvensson,
      author         = "Heller, Michal P. and Svensson, Viktor",
      title          = "{work in progress}"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% anisotropic hydrodynamics for cold atoms

@article{Schaefer:2014awa,
      author         = "Schaefer, Thomas",
      title          = "{Fluid Dynamics and Viscosity in Strongly Correlated
                        Fluids}",
      journal        = "Ann. Rev. Nucl. Part. Sci.",
      volume         = "64",
      year           = "2014",
      pages          = "125-148",
      doi            = "10.1146/annurev-nucl-102313-025439",
      eprint         = "1403.0653",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1403.0653;%%"
}

@article{Bluhm:2015raa,
      author         = "Bluhm, Marcus and Schaefer, Thomas",
      title          = "{Dissipative fluid dynamics for the dilute Fermi gas at
                        unitarity: Anisotropic fluid dynamics}",
      journal        = "Phys. Rev.",
      volume         = "A92",
      year           = "2015",
      number         = "4",
      pages          = "043602",
      doi            = "10.1103/PhysRevA.92.043602",
      eprint         = "1505.00846",
      archivePrefix  = "arXiv",
      primaryClass   = "cond-mat.quant-gas",
      SLACcitation   = "%%CITATION = ARXIV:1505.00846;%%"
}

@article{Bluhm:2015bzi,
      author         = "Bluhm, Marcus and Schaefer, Thomas",
      title          = "{Model-independent determination of the shear viscosity
                        of a trapped unitary Fermi gas: Application to high
                        temperature data}",
      journal        = "Phys. Rev. Lett.",
      volume         = "116",
      year           = "2016",
      number         = "11",
      pages          = "115301",
      doi            = "10.1103/PhysRevLett.116.115301",
      eprint         = "1512.00862",
      archivePrefix  = "arXiv",
      primaryClass   = "cond-mat.quant-gas",
      SLACcitation   = "%%CITATION = ARXIV:1512.00862;%%"
}

@article{Schaefer:2016yzd,
      author         = "Schaefer, Thomas",
      title          = "{A generalized Theory of Diffusion based on Kinetic
                        Theory}",
      year           = "2016",
      eprint         = "1608.05083",
      archivePrefix  = "arXiv",
      primaryClass   = "cond-mat.quant-gas",
      SLACcitation   = "%%CITATION = ARXIV:1608.05083;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% projection method

@article{Florkowski:2011jg,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw",
      title          = "{Projection method for boost-invariant and cylindrically
                        symmetric dissipative hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C85",
      year           = "2012",
      pages          = "044902",
      doi            = "10.1103/PhysRevC.85.044902",
      eprint         = "1111.5997",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1111.5997;%%"
}

@article{Tinti:2013vba,
      author         = "Tinti, Leonardo and Florkowski, Wojciech",
      title          = "{Projection method and new formulation of leading-order
                        anisotropic hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C89",
      year           = "2014",
      number         = "3",
      pages          = "034907",
      doi            = "10.1103/PhysRevC.89.034907",
      eprint         = "1312.6614",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1312.6614;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% shocks

@article{Fogaca:2013cma,
      author         = "FogaÃa, D. A. and Navarra, F. S. and Ferreira Filho, L.
                        G.",
      title          = "{Viscosity, wave damping and shock wave formation in cold
                        hadronic matter}",
      journal        = "Phys. Rev.",
      volume         = "C88",
      year           = "2013",
      number         = "2",
      pages          = "025208",
      doi            = "10.1103/PhysRevC.88.025208",
      eprint         = "1305.0798",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1305.0798;%%"
}

@article{Fogaca:2014gwa,
      author         = "Fogaca, D. A. and Marrochio, H. and Navarra, F. S. and
                        Noronha, J.",
      title          = "{Nonlinear waves in second order conformal
                        hydrodynamics}",
      journal        = "Nucl. Phys.",
      volume         = "A934",
      year           = "2014",
      pages          = "18-40",
      doi            = "10.1016/j.nuclphysa.2014.11.009",
      eprint         = "1402.5548",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1402.5548;%%"
}





%%%%%%%%%%%%
%%%%% small systems

@article{Bozek:2011if,
     author         = "Bozek, Piotr",
     title          = "{Collective flow in p-Pb and d-Pd collisions at TeV
                       energies}",
     journal        = "Phys. Rev.",
     volume         = "C85",
     year           = "2012",
     pages          = "014911",
     doi            = "10.1103/PhysRevC.85.014911",
     eprint         = "1112.0915",
     archivePrefix  = "arXiv",
     primaryClass   = "hep-ph",
     SLACcitation   = "%%CITATION = ARXIV:1112.0915;%%"
}


@article{Habich:2015rtj,
      author         = "Habich, M. and Miller, G. A. and Romatschke, P. and
                        Xiang, W.",
      title          = "{Testing Hydrodynamic Descriptions of of p+p Collisions
                        at $\sqrt{s}=7$ TeV}",
      year           = "2015",
      eprint         = "1512.05354",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1512.05354;%%"
}


@article{Spalinski:2016fnj,
      author         = "Spalinski, Michal",
      title          = "{Small systems and regulator dependence in relativistic
                        hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "8",
      pages          = "085002",
      doi            = "10.1103/PhysRevD.94.085002",
      eprint         = "1607.06381",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1607.06381;%%"
}



@ARTICLE{2013arXiv1308.4453Y,
   author = {{Yamada}, H.~S. and {Ikeda}, K.~S.},
    title = "{A Numerical Test of Pade Approximation for Some Functions with singularity}",
archivePrefix = "arXiv",
   eprint = {1308.4453},
 primaryClass = "math-ph",
 }


@article{Basar:2015ava,
      author         = "Basar, Gokce and Dunne, Gerald V.",
      title          = "{Hydrodynamics, resurgence, and transasymptotics}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "12",
      pages          = "125011",
      doi            = "10.1103/PhysRevD.92.125011",
      eprint         = "1509.05046",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1509.05046;%%"
}


%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% other systems

@article{Brewer:2015ipa,
      author         = "Brewer, Jasmine and Romatschke, Paul",
      title          = "{Nonhydrodynamic Transport in Trapped Unitary Fermi
                        Gases}",
      journal        = "Phys. Rev. Lett.",
      volume         = "115",
      year           = "2015",
      number         = "19",
      pages          = "190404",
      doi            = "10.1103/PhysRevLett.115.190404",
      eprint         = "1508.01199",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1508.01199;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  AdS/CFT

@article{Nickel:2010pr,
      author         = "Nickel, Dominik and Son, Dam T.",
      title          = "{Deconstructing holographic liquids}",
      journal        = "New J. Phys.",
      volume         = "13",
      year           = "2011",
      pages          = "075010",
      doi            = "10.1088/1367-2630/13/7/075010",
      eprint         = "1009.3094",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "INT-PUB-10-041",
      SLACcitation   = "%%CITATION = ARXIV:1009.3094;%%"
}

@article{Bardeen:1973gs,
      author         = "Bardeen, James M. and Carter, B. and Hawking, S. W.",
      title          = "{The Four laws of black hole mechanics}",
      journal        = "Commun. Math. Phys.",
      volume         = "31",
      year           = "1973",
      pages          = "161-170",
      doi            = "10.1007/BF01645742",
      SLACcitation   = "%%CITATION = CMPHA,31,161;%%"
}


@article{Bekenstein:1974ax,
      author         = "Bekenstein, Jacob D.",
      title          = "{Generalized second law of thermodynamics in black hole
                        physics}",
      journal        = "Phys. Rev.",
      volume         = "D9",
      year           = "1974",
      pages          = "3292-3300",
      doi            = "10.1103/PhysRevD.9.3292",
      SLACcitation   = "%%CITATION = PHRVA,D9,3292;%%"
}


@article{Bekenstein:1973ur,
      author         = "Bekenstein, Jacob D.",
      title          = "{Black holes and entropy}",
      journal        = "Phys. Rev.",
      volume         = "D7",
      year           = "1973",
      pages          = "2333-2346",
      doi            = "10.1103/PhysRevD.7.2333",
      SLACcitation   = "%%CITATION = PHRVA,D7,2333;%%"
}

@article{Hawking:1976de,
      author         = "Hawking, S. W.",
      title          = "{Black Holes and Thermodynamics}",
      journal        = "Phys. Rev.",
      volume         = "D13",
      year           = "1976",
      pages          = "191-197",
      doi            = "10.1103/PhysRevD.13.191",
      SLACcitation   = "%%CITATION = PHRVA,D13,191;%%"
}

@article{Hawking:1974sw,
      author         = "Hawking, S. W.",
      title          = "{Particle Creation by Black Holes}",
      booktitle      = "{In *Gibbons, G.W. (ed.), Hawking, S.W. (ed.): Euclidean
                        quantum gravity* 167-188}",
      journal        = "Commun. Math. Phys.",
      volume         = "43",
      year           = "1975",
      pages          = "199-220",
      doi            = "10.1007/BF02345020",
      note           = "[,167(1975)]",
      SLACcitation   = "%%CITATION = CMPHA,43,199;%%"
}

@article{Gubser:1998nz,
      author         = "Gubser, Steven S. and Klebanov, Igor R. and Tseytlin,
                        Arkady A.",
      title          = "{Coupling constant dependence in the thermodynamics of
                        N=4 supersymmetric Yang-Mills theory}",
      journal        = "Nucl. Phys.",
      volume         = "B534",
      year           = "1998",
      pages          = "202-222",
      doi            = "10.1016/S0550-3213(98)00514-8",
      eprint         = "hep-th/9805156",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IASSNS-HEP-98-47, PUPT-1794, IMPERIAL-TP-97-98-47",
      SLACcitation   = "%%CITATION = HEP-TH/9805156;%%"
}

@article{Witten:1998zw,
      author         = "Witten, Edward",
      title          = "{Anti-de Sitter space, thermal phase transition, and
                        confinement in gauge theories}",
      journal        = "Adv. Theor. Math. Phys.",
      volume         = "2",
      year           = "1998",
      pages          = "505-532",
      eprint         = "hep-th/9803131",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IASSNS-HEP-98-21",
      SLACcitation   = "%%CITATION = HEP-TH/9803131;%%"
}


@Article{ Maldacena:1997re,
	archiveprefix = "arXiv",
	author = "Juan Martin Maldacena",
	eprint = "hep-th/9711200",
	journal = "Adv.Theor.Math.Phys.",
	pages = "231--252",
	primaryclass = "hep-th",
	reportnumber = "HUTP-97-A097",
	slaccitation = "%\%CITATION = HEP-TH/9711200;\%\%",
	title = "{The Large N limit of superconformal field theories and supergravity}",
	volume = "2",
	year = "1998"
}

@Article{ Gubser:1998bc,
	archiveprefix = "arXiv",
	author = "S.S. Gubser and Igor R. Klebanov and Alexander M. Polyakov",
	doi = "10.1016/S0370-2693(98)00377-3",
	eprint = "hep-th/9802109",
	journal = "Phys.Lett.",
	pages = "105--114",
	primaryclass = "hep-th",
	reportnumber = "PUPT-1767",
	slaccitation = "%\%CITATION = HEP-TH/9802109;\%\%",
	title = "{Gauge theory correlators from noncritical string theory}",
	volume = "B428",
	year = "1998"
}

@Article{ Witten:1998qj,
	archiveprefix = "arXiv",
	author = "Edward Witten",
	eprint = "hep-th/9802150",
	journal = "Adv.Theor.Math.Phys.",
	pages = "253--291",
	primaryclass = "hep-th",
	reportnumber = "IASSNS-HEP-98-15",
	slaccitation = "%\%CITATION = HEP-TH/9802150;\%\%",
	title = "{Anti-de Sitter space and holography}",
	volume = "2",
	year = "1998"
}

@inproceedings{DHoker:2002nbb,
      author         = "D'Hoker, Eric and Freedman, Daniel Z.",
      title          = "{Supersymmetric gauge theories and the AdS / CFT
                        correspondence}",
      booktitle      = "{Strings, Branes and Extra Dimensions: TASI 2001:
                        Proceedings}",
      year           = "2002",
      pages          = "3-158",
      eprint         = "hep-th/0201253",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "UCLA-02-TEP-3, MIT-CTP-3242",
      SLACcitation   = "%%CITATION = HEP-TH/0201253;%%"
}

@article{Casalderrey-Solana:2013aba,
      author         = "Casalderrey-Solana, Jorge and Heller, Michal P. and
                        Mateos, David and van der Schee, Wilke",
      title          = "{From full stopping to transparency in a holographic
                        model of heavy ion collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "111",
      year           = "2013",
      pages          = "181601",
      doi            = "10.1103/PhysRevLett.111.181601",
      eprint         = "1305.4919",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1305.4919;%%"
}

@article{Janik:2005zt,
	Archiveprefix = {arXiv},
	Author = {Janik, Romuald A. and Peschanski, Robert B.},
	Doi = {10.1103/PhysRevD.73.045013},
	Eprint = {hep-th/0512162},
	Journal = {Phys. Rev.},
	Pages = {045013},
	Slaccitation = {%%CITATION = HEP-TH/0512162;%%},
	Title = {{Asymptotic perfect fluid dynamics as a consequence of AdS/CFT}},
	Volume = {D73},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevD.73.045013}}

@article{Janik:2006gp,
      author         = "Janik, Romuald A. and Peschanski, Robert B.",
      title          = "{Gauge/gravity duality and thermalization of a
                        boost-invariant perfect fluid}",
      journal        = "Phys. Rev.",
      volume         = "D74",
      year           = "2006",
      pages          = "046007",
      doi            = "10.1103/PhysRevD.74.046007",
      eprint         = "hep-th/0606149",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0606149;%%"
}


@article{Chesler:2009cy,
      author         = "Chesler, Paul M. and Yaffe, Laurence G.",
      title          = "{Boost invariant flow, black hole formation, and
                        far-from-equilibrium dynamics in N = 4 supersymmetric
                        Yang-Mills theory}",
      journal        = "Phys.Rev.",
      volume         = "D82",
      pages          = "026006",
      doi            = "10.1103/PhysRevD.82.026006",
      year           = "2010",
      eprint         = "0906.4426",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0906.4426;%%",
}

@article{Chesler:2013lia,
      author         = "Chesler, Paul M. and Yaffe, Laurence G.",
      title          = "{Numerical solution of gravitational dynamics in
                        asymptotically anti-de Sitter spacetimes}",
      journal        = "JHEP",
      volume         = "07",
      year           = "2014",
      pages          = "086",
      doi            = "10.1007/JHEP07(2014)086",
      eprint         = "1309.1439",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1309.1439;%%"
}

@article{Grandclement:2007sb,
      author         = "Grandclement, Philippe and Novak, Jerome",
      title          = "{Spectral methods for numerical relativity}",
      journal        = "Living Rev. Rel.",
      volume         = "12",
      year           = "2009",
      pages          = "1",
      doi            = "10.12942/lrr-2009-1",
      eprint         = "0706.2286",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:0706.2286;%%"
}



@article{Chesler:2010bi,
      author         = "Chesler, Paul M. and Yaffe, Laurence G.",
      title          = "{Holography and colliding gravitational shock waves in
                        asymptotically AdS$_5$ spacetime}",
      journal        = "Phys. Rev. Lett.",
      volume         = "106",
      year           = "2011",
      pages          = "021601",
      doi            = "10.1103/PhysRevLett.106.021601",
      eprint         = "1011.3562",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1011.3562;%%"
}

@article{Chesler:2008hg,
      author         = "Chesler, Paul M. and Yaffe, Laurence G.",
      title          = "{Horizon formation and far-from-equilibrium
                        isotropization in supersymmetric Yang-Mills plasma}",
      journal        = "Phys. Rev. Lett.",
      volume         = "102",
      year           = "2009",
      pages          = "211601",
      doi            = "10.1103/PhysRevLett.102.211601",
      eprint         = "0812.2053",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0812.2053;%%"
}


@article{Janik:2006ft,
      author         = "Janik, Romuald A.",
      title          = "{Viscous plasma evolution from gravity using AdS/CFT}",
      journal        = "Phys.Rev.Lett.",
      volume         = "98",
      pages          = "022302",
      doi            = "10.1103/PhysRevLett.98.022302",
      year           = "2007",
      eprint         = "hep-th/0610144",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0610144;%%",
}


@article{Kovtun:2004de,
      author         = "Kovtun, Pavel and Son, Dam T. and Starinets, Andrei O.",
      title          = "{Viscosity in strongly interacting quantum field theories
                        from black hole physics}",
      journal        = "Phys. Rev. Lett.",
      volume         = "94",
      year           = "2005",
      pages          = "111601",
      doi            = "10.1103/PhysRevLett.94.111601",
      eprint         = "hep-th/0405231",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "INT-PUB-04-09, UW-PT-04-04",
      SLACcitation   = "%%CITATION = HEP-TH/0405231;%%"
}



@article{Heller:2007qt,
      author         = "Heller, Michal P. and Janik, Romuald A.",
      title          = "{Viscous hydrodynamics relaxation time from AdS/CFT}",
      journal        = "Phys. Rev.",
      volume         = "D76",
      year           = "2007",
      pages          = "025027",
      doi            = "10.1103/PhysRevD.76.025027",
      eprint         = "hep-th/0703243",
      archivePrefix  = "arXiv",
      primaryClass   = "HEP-TH",
      SLACcitation   = "%%CITATION = HEP-TH/0703243;%%"
}

@article{Romatschke:2015gic,
      author         = "Romatschke, Paul",
      title          = "{Retarded correlators in kinetic theory: branch cuts,
                        poles and hydrodynamic onset transitions}",
      journal        = "Eur. Phys. J.",
      volume         = "C76",
      year           = "2016",
      number         = "6",
      pages          = "352",
      doi            = "10.1140/epjc/s10052-016-4169-7",
      eprint         = "1512.02641",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1512.02641;%%"
}

@article{Heller:2008mb,
      author         = "Heller, Michal P. and Surowka, Piotr and Loganayagam, R.
                        and Spalinski, Michal and Vazquez, Samuel E.",
      title          = "{Consistent Holographic Description of Boost-Invariant
                        Plasma}",
      journal        = "Phys. Rev. Lett.",
      volume         = "102",
      year           = "2009",
      pages          = "041601",
      doi            = "10.1103/PhysRevLett.102.041601",
      eprint         = "0805.3774",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0805.3774;%%"
}

@article{Nakamura:2006ih,
      author         = "Nakamura, Shin and Sin, Sang-Jin",
      title          = "{A Holographic dual of hydrodynamics}",
      journal        = "JHEP",
      volume         = "09",
      year           = "2006",
      pages          = "020",
      doi            = "10.1088/1126-6708/2006/09/020",
      eprint         = "hep-th/0607123",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = HEP-TH/0607123;%%"
}

@article{Kovtun:2005ev,
      author         = "Kovtun, Pavel K. and Starinets, Andrei O.",
      title          = "{Quasinormal modes and holography}",
      journal        = "Phys. Rev.",
      volume         = "D72",
      year           = "2005",
      pages          = "086009",
      doi            = "10.1103/PhysRevD.72.086009",
      eprint         = "hep-th/0506184",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "NSF-KITP-05-41",
      SLACcitation   = "%%CITATION = HEP-TH/0506184;%%"
}

@inproceedings{Stephanov:2017wlw,
      author         = "Stephanov, Mikhail~A. and Yin, Y.",
      title          = "{Hydrodynamics and critical slowing down}",
      url            = "https://inspirehep.net/record/1594939/files/arXiv:1704.07396.pdf",
      year           = "2017",
      eprint         = "1704.07396",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1704.07396;%%"
}

@article{Landsteiner:2016led,
      author         = "Landsteiner, Karl",
      title          = "{Notes on Anomaly Induced Transport}",
      booktitle      = "{Proceedings, 56th Cracow School of Theoretical Physics :
                        A Panorama of Holography: Zakopane, Poland, May 24-June 1,
                        2016}",
      journal        = "Acta Phys. Polon.",
      volume         = "B47",
      year           = "2016",
      pages          = "2617",
      doi            = "10.5506/APhysPolB.47.2617",
      eprint         = "1610.04413",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IFT-UAM-CSIC-16-103",
      SLACcitation   = "%%CITATION = ARXIV:1610.04413;%%"
}

@article{Buchel:2015saa,
      author         = "Buchel, Alex and Heller, Michal P. and Myers, Robert C.",
      title          = "{Equilibration rates in a strongly coupled nonconformal
                        quark-gluon plasma}",
      journal        = "Phys. Rev. Lett.",
      volume         = "114",
      year           = "2015",
      number         = "25",
      pages          = "251601",
      doi            = "10.1103/PhysRevLett.114.251601",
      eprint         = "1503.07114",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1503.07114;%%"
}

@article{Janik:2015waa,
      author         = "Janik, Romuald A. and Plewa, Grzegorz and Soltanpanahi,
                        Hesam and Spalinski, Michal",
      title          = "{Linearized nonequilibrium dynamics in nonconformal
                        plasma}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "12",
      pages          = "126013",
      doi            = "10.1103/PhysRevD.91.126013",
      eprint         = "1503.07149",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1503.07149;%%"
}

@article{Janik:2016btb,
      author         = "Janik, Romuald A. and Jankowski, Jakub and Soltanpanahi,
                        Hesam",
      title          = "{Quasinormal modes and the phase structure of strongly
                        coupled matter}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2016",
      pages          = "047",
      doi            = "10.1007/JHEP06(2016)047",
      eprint         = "1603.05950",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1603.05950;%%"
}

@article{deHaro:2000vlm,
      author         = "de Haro, Sebastian and Solodukhin, Sergey N. and
                        Skenderis, Kostas",
      title          = "{Holographic reconstruction of space-time and
                        renormalization in the AdS / CFT correspondence}",
      journal        = "Commun. Math. Phys.",
      volume         = "217",
      year           = "2001",
      pages          = "595-622",
      doi            = "10.1007/s002200100381",
      eprint         = "hep-th/0002230",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "SPIN-2000-05, ITP-UU-00-03, PUTP-1921",
      SLACcitation   = "%%CITATION = HEP-TH/0002230;%%"
}

@article{Camanho:2014apa,
      author         = "Camanho, Xian O. and Edelstein, Jose D. and Maldacena,
                        Juan and Zhiboedov, Alexander",
      title          = "{Causality Constraints on Corrections to the Graviton
                        Three-Point Coupling}",
      journal        = "JHEP",
      volume         = "02",
      year           = "2016",
      pages          = "020",
      doi            = "10.1007/JHEP02(2016)020",
      eprint         = "1407.5597",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1407.5597;%%"
}

@article{Myers:1987yn,
      author         = "Myers, Robert C.",
      title          = "{Higher Derivative Gravity, Surface Terms and String
                        Theory}",
      journal        = "Phys. Rev.",
      volume         = "D36",
      year           = "1987",
      pages          = "392",
      doi            = "10.1103/PhysRevD.36.392",
      reportNumber   = "NSF-ITP-87-16",
      SLACcitation   = "%%CITATION = PHRVA,D36,392;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    thermalization


@article{Heller:2011ju,
      author         = "Heller, Michal P. and Janik, Romuald A. and Witaszczyk,
                        Przemyslaw",
      title          = "{The characteristics of thermalization of boost-invariant
                        plasma from holography}",
      journal        = "Phys.Rev.Lett.",
      volume         = "108",
      pages          = "201602",
      doi            = "10.1103/PhysRevLett.108.201602",
      year           = "2012",
      eprint         = "1103.3452",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1103.3452;%%",
}


@article{Heller:2012je,
      author         = "Heller, Michal P. and Janik, Romuald A. and Witaszczyk,
                        Przemyslaw",
      title          = "{A numerical relativity approach to the initial value
                        problem in asymptotically Anti-de Sitter spacetime for
                        plasma thermalization - an ADM formulation}",
      journal        = "Phys.Rev.",
      volume         = "D85",
      pages          = "126002",
      doi            = "10.1103/PhysRevD.85.126002",
      year           = "2012",
      eprint         = "1203.0755",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1203.0755;%%",
}


@article{Jankowski:2014lna,
      author         = "Jankowski, Jakub and Plewa, Grzegorz and Spalinski,
                        Michal",
      title          = "{Statistics of thermalization in Bjorken Flow}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2014",
      pages          = "105",
      doi            = "10.1007/JHEP12(2014)105",
      eprint         = "1411.1969",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1411.1969;%%"
}

@article{Cardoso:2014uka,
      author         = "Cardoso, Vitor and Gualtieri, Leonardo and Herdeiro,
                        Carlos and Sperhake, Ulrich",
      title          = "{Exploring New Physics Frontiers Through Numerical
                        Relativity}",
      journal        = "Living Rev. Relativity",
      volume         = "18",
      year           = "2015",
      pages          = "1",
      doi            = "10.12942/lrr-2015-1, 10.1007/lrr-2015-1",
      eprint         = "1409.0014",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:1409.0014;%%"
}



@article{Bhattacharyya:2008jc,
      author         = "Bhattacharyya, Sayantani and Hubeny, Veronika E and Minwalla, Shiraz and Rangamani, Mukund",
      title          = "{Nonlinear Fluid Dynamics from Gravity}",
      journal        = "JHEP",
      volume         = "0802",
      pages          = "045",
      doi            = "10.1088/1126-6708/2008/02/045",
      year           = "2008",
      eprint         = "0712.2456",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "TIFR-TH-07-44, DCPT-07-73, NI07097",
      SLACcitation   = "%%CITATION = ARXIV:0712.2456;%%",
}

@article{Bhattacharyya:2008xc,
      author         = "Bhattacharyya, Sayantani and Hubeny, Veronika E. and
                        Loganayagam, R. and Mandal, Gautam and Minwalla, Shiraz
                        and Morita, Takeshi and Rangamani, Mukund and Reall,
                        Harvey S.",
      title          = "{Local Fluid Dynamical Entropy from Gravity}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2008",
      pages          = "055",
      doi            = "10.1088/1126-6708/2008/06/055",
      eprint         = "0803.2526",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0803.2526;%%"
}


@article{Plewa:2013rga,
      author         = "Plewa, Grzegorz and Spalinski, Michal",
      title          = "{Entropy currents from holography in hydrodynamics with
                        charge}",
      journal        = "JHEP",
      volume         = "07",
      year           = "2013",
      pages          = "062",
      doi            = "10.1007/JHEP07(2013)062",
      eprint         = "1304.6705",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1304.6705;%%"
}

@article{Plewa:2012vt,
      author         = "Plewa, Grzegorz and Spalinski, Michal",
      title          = "{On the gravity dual of strongly coupled charged plasma}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2013",
      pages          = "002",
      doi            = "10.1007/JHEP05(2013)002",
      eprint         = "1212.2344",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1212.2344;%%"
}

@article{Booth:2011qy,
      author         = "Booth, Ivan and Heller, Michal P. and Plewa, Grzegorz and
                        Spalinski, Michal",
      title          = "{On the apparent horizon in fluid-gravity duality}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "106005",
      doi            = "10.1103/PhysRevD.83.106005",
      eprint         = "1102.2885",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1102.2885;%%"
}

@article{Booth:2010kr,
      author         = "Booth, Ivan and Heller, Michal P. and Spalinski, Michal",
      title          = "{Black Brane Entropy and Hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "061901",
      doi            = "10.1103/PhysRevD.83.061901",
      eprint         = "1010.6301",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1010.6301;%%"
}

@article{Booth:2009ct,
      author         = "Booth, Ivan and Heller, Michal P. and Spalinski, Michal",
      title          = "{Black brane entropy and hydrodynamics: The
                        Boost-invariant case}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "126013",
      doi            = "10.1103/PhysRevD.80.126013",
      eprint         = "0910.0748",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0910.0748;%%"
}




%%%%
%% Nonhydro modes
%%%

@article{Lewis:2016uei,
      author         = "Lewis, William E. and Romatschke, Paul",
      title          = "{Higher-Harmonic Collective Modes in a Trapped Gas from
                        Second-Order Hydrodynamics}",
      journal        = "New J. Phys.",
      volume         = "19",
      year           = "2017",
      number         = "2",
      pages          = "023042",
      doi            = "10.1088/1367-2630/aa5d6a",
      eprint         = "1610.01611",
      archivePrefix  = "arXiv",
      primaryClass   = "cond-mat.quant-gas",
      SLACcitation   = "%%CITATION = ARXIV:1610.01611;%%"
}


@article{Beuf:2009cx,
      author         = "Beuf, Guillaume and Heller, Michal P. and Janik, Romuald
                        A. and Peschanski, Robi",
      title          = "{Boost-invariant early time dynamics from AdS/CFT}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2009",
      pages          = "043",
      doi            = "10.1088/1126-6708/2009/10/043",
      eprint         = "0906.4423",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0906.4423;%%"
}

%%%%%%%%%%%%%%%%%%%%%%%%%
% color-tubes papers


@article{Bialas:1984wv,
      author         = "Bialas, Andrzej and Czyz, Wieslaw",
      title          = "{Boost Invariant Boltzmann-vlasov Equations for
                        Relativistic Quark - Anti-quark Plasma}",
      journal        = "Phys. Rev.",
      volume         = "D30",
      year           = "1984",
      pages          = "2371",
      doi            = "10.1103/PhysRevD.30.2371",
      reportNumber   = "MPI-PAE/PTh 30/84",
      SLACcitation   = "%%CITATION = PHRVA,D30,2371;%%"
}

@article{Bialas:1987en,
      author         = "Bialas, Andrzej and Czyz, Wieslaw and Dyrek, Andrzej and Florkowski, Wojciech",
      title          = "{Oscillations of Quark - Gluon Plasma Generated in Strong
                        Color Fields}",
      journal        = "Nucl. Phys.",
      volume         = "B296",
      year           = "1988",
      pages          = "611-624",
      doi            = "10.1016/0550-3213(88)90035-1",
      reportNumber   = "TPJU-3/87",
      SLACcitation   = "%%CITATION = NUPHA,B296,611;%%"
}

@article{Banerjee:1989by,
      author         = "Banerjee, Bakul and Bhalerao, Rajeev~S. and Ravishankar, V.",
      title          = "{Equilibration of the Quark - Gluon Plasma Produced in
                        Relativistic Heavy Ion Collisions}",
      journal        = "Phys. Lett.",
      volume         = "B224",
      year           = "1989",
      pages          = "16-20",
      doi            = "10.1016/0370-2693(89)91041-1",
      reportNumber   = "TIFR/TH/89-2",
      SLACcitation   = "%%CITATION = PHLTA,B224,16;%%"
}

@article{Florkowski:2016qig,
      author         = "Florkowski, Wojciech and Ryblewski, Radoslaw",
      title          = "{Separation of elastic and inelastic processes in the
                        relaxation-time approximation for the collision integral}",
      journal        = "Phys. Rev.",
      volume         = "C93",
      year           = "2016",
      number         = "6",
      pages          = "064903",
      doi            = "10.1103/PhysRevC.93.064903",
      eprint         = "1603.01704",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1603.01704;%%"
}



%%%%%%%%%%%%%%%%%%%%%%%%%
% other papers

@article{tHooft:1973alw,
      author         = "'t Hooft, Gerard",
      title          = "{A Planar Diagram Theory for Strong Interactions}",
      journal        = "Nucl. Phys.",
      volume         = "B72",
      year           = "1974",
      pages          = "461",
      doi            = "10.1016/0550-3213(74)90154-0",
      reportNumber   = "CERN-TH-1786",
      SLACcitation   = "%%CITATION = NUPHA,B72,461;%%"
}


%% added by WF on June 15

@article{Muronga:2001zk,
      author         = "Muronga, Azwinndini",
      title          = "{Second order dissipative fluid dynamics for
                        ultrarelativistic nuclear collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "88",
      year           = "2002",
      pages          = "062302",
      doi            = "10.1103/PhysRevLett.88.062302",
      note           = "[Erratum: Phys. Rev. Lett.89,159901(2002)]",
      eprint         = "nucl-th/0104064",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "NUC-MINN-01-8-T",
      SLACcitation   = "%%CITATION = NUCL-TH/0104064;%%"
}

@article{Muronga:2003ta,
      author         = "Muronga, Azwinndini",
      title          = "{Causal theories of dissipative relativistic fluid
                        dynamics for nuclear collisions}",
      journal        = "Phys. Rev.",
      volume         = "C69",
      year           = "2004",
      pages          = "034903",
      doi            = "10.1103/PhysRevC.69.034903",
      eprint         = "nucl-th/0309055",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0309055;%%"
}


@article{Itakura:2007mx,
      author         = "Itakura, Kazunori and Morimatsu, Osamu and Otomo,
                        Hiroshi",
      title          = "{Shear viscosity of a hadronic gas mixture}",
      journal        = "Phys. Rev.",
      volume         = "D77",
      year           = "2008",
      pages          = "014014",
      doi            = "10.1103/PhysRevD.77.014014",
      eprint         = "0711.1034",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0711.1034;%%"
}

@article{Bozek:2009dw,
      author         = "Bozek, Piotr",
      title          = "{Bulk and shear viscosities of matter created in
                        relativistic heavy-ion collisions}",
      journal        = "Phys. Rev.",
      volume         = "C81",
      year           = "2010",
      pages          = "034909",
      doi            = "10.1103/PhysRevC.81.034909",
      eprint         = "0911.2397",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:0911.2397;%%"
}

@article{Bluhm:2010qf,
      author         = "Bluhm, Marcus and Kampfer, Burkhard and Redlich, Krzysztof",
      title          = "{Bulk and shear viscosities of the gluon plasma in a
                        quasiparticle description}",
      journal        = "Phys. Rev.",
      volume         = "C84",
      year           = "2011",
      pages          = "025201",
      doi            = "10.1103/PhysRevC.84.025201",
      eprint         = "1011.5634",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1011.5634;%%"
}


@article{Shen:2014vra,
      author         = "Shen, Chun and Qiu, Zhi and Song, Huichao and Bernhard,
                        Jonah and Bass, Steffen and Heinz, Ulrich",
      title          = "{The iEBE-VISHNU code package for relativistic heavy-ion
                        collisions}",
      journal        = "Comput. Phys. Commun.",
      volume         = "199",
      year           = "2016",
      pages          = "61-85",
      doi            = "10.1016/j.cpc.2015.08.039",
      eprint         = "1409.8164",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1409.8164;%%"
}


@article{Pratt:2015zsa,
      author         = "Pratt, Scott and Sangaline, Evan and Sorensen, Paul and
                        Wang, Hui",
      title          = "{Constraining the Eq. of State of Super-Hadronic Matter
                        from Heavy-Ion Collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "114",
      year           = "2015",
      pages          = "202301",
      doi            = "10.1103/PhysRevLett.114.202301",
      eprint         = "1501.04042",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1501.04042;%%"
}

@inproceedings{Bass:2017zyn,
      author         = "Bass, Steffen A. and Bernhard, Jonah E. and Moreland, J.
                        Scott",
      title          = "{Determination of Quark-Gluon-Plasma Parameters from a
                        Global Bayesian Analysis}",
      booktitle      = "{26th International Conference on Ultrarelativistic
                        Nucleus-Nucleus Collisions (Quark Matter 2017)
                        Chicago,Illinois, USA, February 6-11, 2017}",
      url            = "https://inspirehep.net/record/1594915/files/arXiv:1704.07671.pdf",
      year           = "2017",
      eprint         = "1704.07671",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1704.07671;%%"
}



@article{Tinti:2016bav,
      author         = "Tinti, Leonardo and Jaiswal, Amaresh and Ryblewski,
                        Radoslaw",
      title          = "{Quasiparticle second-order viscous hydrodynamics from
                        kinetic theory}",
      journal        = "Phys. Rev.",
      volume         = "D95",
      year           = "2017",
      number         = "5",
      pages          = "054007",
      doi            = "10.1103/PhysRevD.95.054007",
      eprint         = "1612.07329",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1612.07329;%%"
}


@article{Alqahtani:2017jwl,
      author         = "Alqahtani, Mubarak and Nopoush, Mohammad and Ryblewski,
                        Radoslaw and Strickland, Michael",
      title          = "{(3+1)D Quasiparticle Anisotropic Hydrodynamics for
                        Ultrarelativistic Heavy-Ion Collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "119",
      year           = "2017",
      number         = "4",
      pages          = "042301",
      doi            = "10.1103/PhysRevLett.119.042301",
      eprint         = "1703.05808",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1703.05808;%%"
}


@article{Borsanyi:2010cj,
      author         = "Borsanyi, Szabolcs and Endrodi, Gergely and Fodor, Zoltan
                        and Jakovac, Antal and Katz, Sandor D. and Krieg, Stefan
                        and Ratti, Claudia and Szabo, Kalman K.",
      title          = "{The QCD equation of state with dynamical quarks}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2010",
      pages          = "077",
      doi            = "10.1007/JHEP11(2010)077",
      eprint         = "1007.2580",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "WUB-10-12",
      SLACcitation   = "%%CITATION = ARXIV:1007.2580;%%"
}


@article{Jaiswal:2016hex,
      author         = "Jaiswal, Amaresh and Roy, Victor",
      title          = "{Relativistic hydrodynamics in heavy-ion collisions:
                        general aspects and recent developments}",
      journal        = "Adv. High Energy Phys.",
      volume         = "2016",
      year           = "2016",
      pages          = "9623034",
      doi            = "10.1155/2016/9623034",
      eprint         = "1605.08694",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1605.08694;%%"
}

@article{Gelis:2014qga,
      author         = "Gelis, F.",
      title          = "{The Initial Stages of Heavy Ion Collisions}",
      booktitle      = "{54th Cracow School of Theoretical Physics: QCD meets
                        experiment: Zakopane, Poland, June 12-20, 2014}",
      journal        = "Acta Phys. Polon.",
      volume         = "B45",
      year           = "2014",
      number         = "12",
      pages          = "2257-2306",
      doi            = "10.5506/APhysPolB.45.2257",
      SLACcitation   = "%%CITATION = APPOA,B45,2257;%%"
}

@article{Romatschke:2007mq,
      author         = "Romatschke, Paul and Romatschke, Ulrike",
      title          = "{Viscosity Information from Relativistic Nuclear
                        Collisions: How Perfect is the Fluid Observed at RHIC?}",
      journal        = "Phys. Rev. Lett.",
      volume         = "99",
      year           = "2007",
      pages          = "172301",
      doi            = "10.1103/PhysRevLett.99.172301",
      eprint         = "0706.1522",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "INT-PUB-07-14",
      SLACcitation   = "%%CITATION = ARXIV:0706.1522;%%"
}

@article{Heinz:2013th,
      author         = "Heinz, Ulrich and Snellings, Raimond",
      title          = "{Collective flow and viscosity in relativistic heavy-ion
                        collisions}",
      journal        = "Ann. Rev. Nucl. Part. Sci.",
      volume         = "63",
      year           = "2013",
      pages          = "123-151",
      doi            = "10.1146/annurev-nucl-102212-170540",
      eprint         = "1301.2826",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1301.2826;%%"
}

@article{Song:2010mg,
      author         = "Song, Huichao and Bass, Steffen A. and Heinz, Ulrich and
                        Hirano, Tetsufumi and Shen, Chun",
      title          = "{200 A GeV Au+Au collisions serve a nearly perfect
                        quark-gluon liquid}",
      journal        = "Phys. Rev. Lett.",
      volume         = "106",
      year           = "2011",
      pages          = "192301",
      doi            = "10.1103/PhysRevLett.106.192301,
                        10.1103/PhysRevLett.109.139904",
      note           = "[Erratum: Phys. Rev. Lett.109,139904(2012)]",
      eprint         = "1011.2783",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1011.2783;%%"
}

@article{Alver:2010gr,
      author         = "Alver, B. and Roland, G.",
      title          = "{Collision geometry fluctuations and triangular flow in
                        heavy-ion collisions}",
      journal        = "Phys. Rev.",
      volume         = "C81",
      year           = "2010",
      pages          = "054905",
      doi            = "10.1103/PhysRevC.82.039903, 10.1103/PhysRevC.81.054905",
      note           = "[Erratum: Phys. Rev.C82,039903(2010)]",
      eprint         = "1003.0194",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1003.0194;%%"
}

@article{Noronha-Hostler:2013gga,
      author         = "Noronha-Hostler, Jacquelyn and Denicol, Gabriel S. and
                        Noronha, Jorge and Andrade, Rone P. G. and Grassi,
                        Frederique",
      title          = "{Bulk Viscosity Effects in Event-by-Event Relativistic
                        Hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "C88",
      year           = "2013",
      number         = "4",
      pages          = "044916",
      doi            = "10.1103/PhysRevC.88.044916",
      eprint         = "1305.1981",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1305.1981;%%"
}

@article{Anderson:1974a,
      author         = "Anderson,   James~L. and Witting,H.~R.",
      title          = "{A relativistic relaxation-time model for the Boltzmann equation}",
      journal        = "  Physica",
      volume         = "74",
      year           = "1974",
      number         = "",
      pages          = "466",
}

@article{Anderson:1974b,
      author         = "Anderson,   James~L. and Witting,H.~R.",
      title          = "{Relativistic quantum transport coefficients}",
      journal        = "  Physica",
      volume         = "74",
      year           = "1974",
      number         = "",
      pages          = "489",
}

@article{Czyz:1986mr,
      author         = "Czyz, Wieslaw and Florkowski, Wojciech",
      title          = "{Kinetic Coefficients for Quark - Anti-quark Plasma}",
      journal        = "Acta Phys. Polon.",
      volume         = "B17",
      year           = "1986",
      pages          = "819-837",
      reportNumber   = "IFJ-1311-PH",
      SLACcitation   = "%%CITATION = APPOA,B17,819;%%"
}


@article{Berti:2009kk,
      author         = "Berti, Emanuele and Cardoso, Vitor and Starinets, Andrei
                        O.",
      title          = "{Quasinormal modes of black holes and black branes}",
      journal        = "Class. Quant. Grav.",
      volume         = "26",
      year           = "2009",
      pages          = "163001",
      doi            = "10.1088/0264-9381/26/16/163001",
      eprint         = "0905.2975",
      archivePrefix  = "arXiv",
      primaryClass   = "gr-qc",
      SLACcitation   = "%%CITATION = ARXIV:0905.2975;%%"
}

@article{Gelis:2013rba,
      author         = "Epelbaum, Thomas and Gelis, Francois",
      title          = "{Pressure isotropization in high energy heavy ion
                        collisions}",
      journal        = "Phys. Rev. Lett.",
      volume         = "111",
      year           = "2013",
      pages          = "232301",
      doi            = "10.1103/PhysRevLett.111.232301",
      eprint         = "1307.2214",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1307.2214;%%"
}

@article{Berges:2013fga,
      author         = "Berges, Juergen and Boguslavski, Kirill and Schlichting,
                        Soeren and Venugopalan, Raju",
      title          = "{Universal attractor in a highly occupied non-Abelian
                        plasma}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "11",
      pages          = "114007",
      doi            = "10.1103/PhysRevD.89.114007",
      eprint         = "1311.3005",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1311.3005;%%"
}


@book{deGroot:1980,
      author         = "de~Groot, Sybren~R. and van~Leeuwen, Willem~A.  and van~Weert, Christianus~G.",
      title          = "{Relativistic Kinetic Theory: Principles and Applications}",
      journal        = "North-Holland, Amsterdam",
      year           = "1980",
      reportNumber   = "",
      SLACcitation   = ""
}


@article{Broniowski:2008vp,
      author         = "Broniowski, Wojciech and Chojnacki, Mikolaj and
                        Florkowski, Wojciech and Kisiel, Adam",
      title          = "{Uniform Description of Soft Observables in Heavy-Ion
                        Collisions at s(NN)**(1/2) = 200 GeV**2}",
      journal        = "Phys. Rev. Lett.",
      volume         = "101",
      year           = "2008",
      pages          = "022301",
      doi            = "10.1103/PhysRevLett.101.022301",
      eprint         = "0801.4361",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:0801.4361;%%"
}

@article{Schenke:2006yp,
      author         = "Schenke, Bjoern and Strickland, Michael",
      title          = "{Photon production from an anisotropic quark-gluon
                        plasma}",
      journal        = "Phys. Rev.",
      volume         = "D76",
      year           = "2007",
      pages          = "025023",
      doi            = "10.1103/PhysRevD.76.025023",
      eprint         = "hep-ph/0611332",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0611332;%%"
}


@article{McLerran:2014hza,
      author         = "McLerran, Larry~D. and Schenke, Bjoern",
      title          = "{The Glasma, Photons and the Implications of Anisotropy}",
      journal        = "Nucl. Phys.",
      volume         = "A929",
      year           = "2014",
      pages          = "71-82",
      doi            = "10.1016/j.nuclphysa.2014.06.004",
      eprint         = "1403.7462",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1403.7462;%%"
}


@article{Martinez:2008di,
      author         = "Martinez, Mauricio and Strickland, Michael",
      title          = "{Pre-equilibrium dilepton production from an anisotropic
                        quark-gluon plasma}",
      journal        = "Phys. Rev.",
      volume         = "C78",
      year           = "2008",
      pages          = "034917",
      doi            = "10.1103/PhysRevC.78.034917",
      eprint         = "0805.4552",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0805.4552;%%"
}


@article{Shuryak:2012nf,
      author         = "Shuryak, Edward",
      title          = "{Monitoring parton equilibration in heavy ion collisions
                        via dilepton polarization}",
      year           = "2012",
      eprint         = "1203.1012",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1203.1012;%%"
}

@article{Wu:2011yd,
      author         = "Wu, Bin and Romatschke, Paul",
      title          = "{Shock wave collisions in AdS5: approximate numerical
                        solutions}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "C22",
      year           = "2011",
      pages          = "1317-1342",
      doi            = "10.1142/S0129183111016920",
      eprint         = "1108.3715",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1108.3715;%%"
}


@article{Aniceto:2011nu,
      author         = "Aniceto, Ines and Schiappa, Ricardo and Vonk, Marcel",
      title          = "{The Resurgence of Instantons in String Theory}",
      journal        = "Commun. Num. Theor. Phys.",
      volume         = "6",
      year           = "2012",
      pages          = "339-496",
      doi            = "10.4310/CNTP.2012.v6.n2.a3",
      eprint         = "1106.5922",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1106.5922;%%"
}

@article{Grumiller:2008va,
      author         = "Grumiller, Daniel and Romatschke, Paul",
      title          = "{On the collision of two shock waves in AdS(5)}",
      journal        = "JHEP",
      volume         = "08",
      year           = "2008",
      pages          = "027",
      doi            = "10.1088/1126-6708/2008/08/027",
      eprint         = "0803.3226",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "INT-PUB-08-06, MIT-CTP-3939, YITP-08-18",
      SLACcitation   = "%%CITATION = ARXIV:0803.3226;%%"
}


@article{Bhattacharya:2011tra,
      author         = "Bhattacharya, Jyotirmoy and Bhattacharyya, Sayantani and
                        Minwalla, Shiraz and Yarom, Amos",
      title          = "{A Theory of first order dissipative superfluid
                        dynamics}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2014",
      pages          = "147",
      doi            = "10.1007/JHEP05(2014)147",
      eprint         = "1105.3733",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "PUPT-2375",
      SLACcitation   = "%%CITATION = ARXIV:1105.3733;%%"
}

@article{Nunez:2003eq,
      author         = "Nunez, Alvaro and Starinets, Andrei O.",
      title          = "{AdS / CFT correspondence, quasinormal modes, and thermal
                        correlators in N=4 SYM}",
      journal        = "Phys. Rev.",
      volume         = "D67",
      year           = "2003",
      pages          = "124013",
      doi            = "10.1103/PhysRevD.67.124013",
      eprint         = "hep-th/0302026",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "NYU-TH-03-02-01, INT-PUB-03-02",
      SLACcitation   = "%%CITATION = HEP-TH/0302026;%%"
}

@article{Haehl:2014zda,
      author         = "Haehl, Felix M. and Loganayagam, R. and Rangamani,
                        Mukund",
      title          = "{The eightfold way to dissipation}",
      journal        = "Phys. Rev. Lett.",
      volume         = "114",
      year           = "2015",
      pages          = "201601",
      doi            = "10.1103/PhysRevLett.114.201601",
      eprint         = "1412.1090",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DCPT-14-65",
      SLACcitation   = "%%CITATION = ARXIV:1412.1090;%%"
}

@article{Romatschke:2017vte,
      author         = "Romatschke, Paul",
      title          = "{Relativistic Fluid Dynamics Far From Local Equilibrium}",
      journal        = "Phys. Rev. Lett.",
      volume         = "120",
      year           = "2018",
      number         = "1",
      pages          = "012301",
      doi            = "10.1103/PhysRevLett.120.012301",
      eprint         = "1704.08699",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1704.08699;%%"
}

@article{Spalinski:2017mel,
      author         = "Spaliński, Michał",
      title          = "{On the hydrodynamic attractor of Yang–Mills plasma}",
      journal        = "Phys. Lett.",
      volume         = "B776",
      year           = "2018",
      pages          = "468-472",
      doi            = "10.1016/j.physletb.2017.11.059",
      eprint         = "1708.01921",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1708.01921;%%"
}

@article{Strickland:2017kux,
      author         = "Strickland, Michael and Noronha, Jorge and Denicol,
                        Gabriel",
      title          = "{Anisotropic nonequilibrium hydrodynamic attractor}",
      journal        = "Phys. Rev.",
      volume         = "D97",
      year           = "2018",
      number         = "3",
      pages          = "036020",
      doi            = "10.1103/PhysRevD.97.036020",
      eprint         = "1709.06644",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1709.06644;%%"
}


@article{Haehl:2015pja,
      author         = "Haehl, Felix M. and Loganayagam, R. and Rangamani,
                        Mukund",
      title          = "{Adiabatic hydrodynamics: The eightfold way to
                        dissipation}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2015",
      pages          = "060",
      doi            = "10.1007/JHEP05(2015)060",
      eprint         = "1502.00636",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DCPT-15-01",
      SLACcitation   = "%%CITATION = ARXIV:1502.00636;%%"
}

@article{Liddle:1994dx,
      author         = "Liddle, Andrew R. and Parsons, Paul and Barrow, John D.",
      title          = "{Formalizing the slow roll approximation in inflation}",
      journal        = "Phys. Rev.",
      volume         = "D50",
      year           = "1994",
      pages          = "7222-7232",
      doi            = "10.1103/PhysRevD.50.7222",
      eprint         = "astro-ph/9408015",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "SUSSEX-AST-94-8-1",
      SLACcitation   = "%%CITATION = ASTRO-PH/9408015;%%"
}

@article{Lipatov:1976ny,
      author         = "Lipatov, L. N.",
      title          = "{Divergence of the Perturbation Theory Series and the
                        Quasiclassical Theory}",
      journal        = "Sov. Phys. JETP",
      volume         = "45",
      year           = "1977",
      pages          = "216-223",
      note           = "[Zh. Eksp. Teor. Fiz.72,411(1977)]",
      reportNumber   = "LENINGRAD-76-255",
      SLACcitation   = "%%CITATION = SPHJA,45,216;%%"
}

@article{Boyd1999,
    author = {Boyd, J. P.},
    citeulike-article-id = {1166725},
    journal = {Acta Appl. Math},
    keywords = {bibtex-import},
    pages = {1--98},
    title = {{The devil's invention: asymptotic, superasymptotic and hyperasymptotic series}},
    volume = {56},
    year = {1999}
}

@article{Dunne,
      author         = "Dunne, Gerald V.",
      title          = "{Resurgence and Trans-series in Quantum Theories}",
      journal        = "Lectures given at the Schladming Winter School 2015",
}

@article{Aniceto:2013fka,
      author         = "Aniceto, Ines and Schiappa, Ricardo",
      title          = "{Nonperturbative Ambiguities and the Reality of Resurgent
                        Transseries}",
      journal        = "Commun. Math. Phys.",
      volume         = "335",
      year           = "2015",
      number         = "1",
      pages          = "183-245",
      doi            = "10.1007/s00220-014-2165-z",
      eprint         = "1308.1115",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1308.1115;%%"
}

@article{Buchel:2008vz,
      author         = "Buchel, Alex and Myers, Robert C. and Sinha, Aninda",
      title          = "{Beyond eta/s = 1/4 pi}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2009",
      pages          = "084",
      doi            = "10.1088/1126-6708/2009/03/084",
      eprint         = "0812.2521",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "UWO-TH-08-15",
      SLACcitation   = "%%CITATION = ARXIV:0812.2521;%%"
}

@article{Attems:2017zam,
      author         = "Attems, Maximilian and Casalderrey-Solana, Jorge and
                        Mateos, David and Santos-Olivan, Daniel and Sopuerta,
                        Carlos F. and Triana, Miquel and Zilhao, Miguel",
      title          = "{Paths to equilibrium in non-conformal collisions}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2017",
      pages          = "154",
      doi            = "10.1007/JHEP06(2017)154",
      eprint         = "1703.09681",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "ICCUB-17-009",
      SLACcitation   = "%%CITATION = ARXIV:1703.09681;%%"
}


@article{Attems:2016tby,
      author         = "Attems, Maximilian and Casalderrey-Solana, Jorge and
                        Mateos, David and Santos-Olivan, Daniel and Sopuerta,
                        Carlos F. and Triana, Miquel and Zilhao, Miguel",
      title          = "{Holographic Collisions in Non-conformal Theories}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2017",
      pages          = "026",
      doi            = "10.1007/JHEP01(2017)026",
      eprint         = "1604.06439",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "ICCUB-16-013",
      SLACcitation   = "%%CITATION = ARXIV:1604.06439;%%"
}

@article{Buchel:2008uu,
      author         = "Buchel, Alex and Pagnutti, Chris",
      title          = "{Bulk viscosity of N=2* plasma}",
      journal        = "Nucl. Phys.",
      volume         = "B816",
      year           = "2009",
      pages          = "62-72",
      doi            = "10.1016/j.nuclphysb.2009.02.022",
      eprint         = "0812.3623",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "UWO-TH-08-18",
      SLACcitation   = "%%CITATION = ARXIV:0812.3623;%%"
}

@article{Chesler:2016ceu,
      author         = "Chesler, Paul M.",
      title          = "{How big are the smallest drops of quark-gluon plasma?}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2016",
      pages          = "146",
      doi            = "10.1007/JHEP03(2016)146",
      eprint         = "1601.01583",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1601.01583;%%"
}


@article{Chesler:2015wra,
      author         = "Chesler, Paul M. and Yaffe, Laurence G.",
      title          = "{Holography and off-center collisions of localized shock
                        waves}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2015",
      pages          = "070",
      doi            = "10.1007/JHEP10(2015)070",
      eprint         = "1501.04644",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1501.04644;%%"
}


@article{Chesler:2015fpa,
      author         = "Chesler, Paul M. and Kilbertus, Niki and van der Schee,
                        Wilke",
      title          = "{Universal hydrodynamic flow in holographic planar shock
                        collisions}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2015",
      pages          = "135",
      doi            = "10.1007/JHEP11(2015)135",
      eprint         = "1507.02548",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1507.02548;%%"
}


@article{Kovtun:2011np,
      author         = "Kovtun, Pavel and Moore, Guy D. and Romatschke, Paul",
      title          = "{The stickiness of sound: An absolute lower limit on
                        viscosity and the breakdown of second order relativistic
                        hydrodynamics}",
      journal        = "Phys. Rev.",
      volume         = "D84",
      year           = "2011",
      pages          = "025006",
      doi            = "10.1103/PhysRevD.84.025006",
      eprint         = "1104.1586",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1104.1586;%%"
}

@article{Akamatsu:2016llw,
      author         = "Akamatsu, Yukinao and Mazeliauskas, Aleksas and Teaney,
                        Derek",
      title          = "{A kinetic regime of hydrodynamic fluctuations and long
                        time tails for a Bjorken expansion}",
      journal        = "Phys. Rev.",
      volume         = "C95",
      year           = "2017",
      number         = "1",
      pages          = "014909",
      doi            = "10.1103/PhysRevC.95.014909",
      eprint         = "1606.07742",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1606.07742;%%"
}


@article{Ishii:2015gia,
      author         = "Ishii, Takaaki and Kiritsis, Elias and Rosen,
                        Christopher",
      title          = "{Thermalization in a Holographic Confining Gauge Theory}",
      journal        = "JHEP",
      volume         = "08",
      year           = "2015",
      pages          = "008",
      doi            = "10.1007/JHEP08(2015)008",
      eprint         = "1503.07766",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CCTP-2015-08, CCQCN-2015-67",
      SLACcitation   = "%%CITATION = ARXIV:1503.07766;%%"
}


@article{Figueras:2009iu,
      author         = "Figueras, Pau and Hubeny, Veronika E. and Rangamani,
                        Mukund and Ross, Simon F.",
      title          = "{Dynamical black holes and expanding plasmas}",
      journal        = "JHEP",
      volume         = "04",
      year           = "2009",
      pages          = "137",
      doi            = "10.1088/1126-6708/2009/04/137",
      eprint         = "0902.4696",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DCPT-09-13, NSF-KITP-09-20",
      SLACcitation   = "%%CITATION = ARXIV:0902.4696;%%"
}


@article{Grozdanov:2016fkt,
      author         = "Grozdanov, Saso and Starinets, Andrei O.",
      title          = "{Second-order transport, quasinormal modes and
                        zero-viscosity limit in the Gauss-Bonnet holographic
                        fluid}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2017",
      pages          = "166",
      doi            = "10.1007/JHEP03(2017)166",
      eprint         = "1611.07053",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-16-21P",
      SLACcitation   = "%%CITATION = ARXIV:1611.07053;%%"
}


@article{Grozdanov:2016vgg,
      author         = "Grozdanov, Saso and Kaplis, Nikolaos and Starinets,
                        Andrei O.",
      title          = "{From strong to weak coupling in holographic models of
                        thermalization}",
      journal        = "JHEP",
      volume         = "07",
      year           = "2016",
      pages          = "151",
      doi            = "10.1007/JHEP07(2016)151",
      eprint         = "1605.02173",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "OUTP-16-11P, INT-PUB-15-076",
      SLACcitation   = "%%CITATION = ARXIV:1605.02173;%%"
}


@article{Buchel:2016cbj,
      author         = "Buchel, Alex and Heller, Michal P. and Noronha, Jorge",
      title          = "{Entropy Production, Hydrodynamics, and Resurgence in the
                        Primordial Quark-Gluon Plasma from Holography}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "10",
      pages          = "106011",
      doi            = "10.1103/PhysRevD.94.106011",
      eprint         = "1603.05344",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1603.05344;%%"
}

@article{Kinoshita:2008dq,
      author         = "Kinoshita, Shunichiro and Mukohyama, Shinji and Nakamura,
                        Shin and Oda, Kin-ya",
      title          = "{A Holographic Dual of Bjorken Flow}",
      journal        = "Prog. Theor. Phys.",
      volume         = "121",
      year           = "2009",
      pages          = "121-164",
      doi            = "10.1143/PTP.121.121",
      eprint         = "0807.3797",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CQUEST-2008-0201, IPMU-08-0039, OU-HET-601-2008,
                        UTAP-601",
      SLACcitation   = "%%CITATION = ARXIV:0807.3797;%%"
}

@article{Kinoshita:2009dx,
      author         = "Kinoshita, Shunichiro and Mukohyama, Shinji and Nakamura,
                        Shin and Oda, Kin-ya",
      title          = "{Consistent Anti-de Sitter-Space/Conformal-Field-Theory
                        Dual for a Time-Dependent Finite Temperature System}",
      journal        = "Phys. Rev. Lett.",
      volume         = "102",
      year           = "2009",
      pages          = "031601",
      doi            = "10.1103/PhysRevLett.102.031601",
      eprint         = "0901.4834",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CQUEST-2008-0203, IPMU-08-0055, OU-HET-609-2008,
                        UTAP-603",
      SLACcitation   = "%%CITATION = ARXIV:0901.4834;%%"
}


@article{Bhattacharyya:2008mz,
      author         = "Bhattacharyya, Sayantani and Loganayagam, R. and Mandal,
                        Ipsita and Minwalla, Shiraz and Sharma, Ankit",
      title          = "{Conformal Nonlinear Fluid Dynamics from Gravity in
                        Arbitrary Dimensions}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2008",
      pages          = "116",
      doi            = "10.1088/1126-6708/2008/12/116",
      eprint         = "0809.4272",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "TIFR-TH-08-38",
      SLACcitation   = "%%CITATION = ARXIV:0809.4272;%%"
}

@article{Loganayagam:2008is,
      author         = "Loganayagam, R.",
      title          = "{Entropy Current in Conformal Hydrodynamics}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2008",
      pages          = "087",
      doi            = "10.1088/1126-6708/2008/05/087",
      eprint         = "0801.3701",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0801.3701;%%"
}

@article{Kats:2007mq,
      author         = "Kats, Yevgeny and Petrov, Pavel",
      title          = "{Effect of curvature squared corrections in AdS on the
                        viscosity of the dual gauge theory}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2009",
      pages          = "044",
      doi            = "10.1088/1126-6708/2009/01/044",
      eprint         = "0712.0743",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:0712.0743;%%"
}

@article{Brigante:2007nu,
      author         = "Brigante, Mauro and Liu, Hong and Myers, Robert C. and
                        Shenker, Stephen and Yaida, Sho",
      title          = "{Viscosity Bound Violation in Higher Derivative Gravity}",
      journal        = "Phys. Rev.",
      volume         = "D77",
      year           = "2008",
      pages          = "126006",
      doi            = "10.1103/PhysRevD.77.126006",
      eprint         = "0712.0805",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "CAS-KITPC-ITP-025, MIT-CTP-3918, SU-ITP-07-22",
      SLACcitation   = "%%CITATION = ARXIV:0712.0805;%%"
}

@article{Brigante:2008gz,
      author         = "Brigante, Mauro and Liu, Hong and Myers, Robert C. and
                        Shenker, Stephen and Yaida, Sho",
      title          = "{The Viscosity Bound and Causality Violation}",
      journal        = "Phys. Rev. Lett.",
      volume         = "100",
      year           = "2008",
      pages          = "191601",
      doi            = "10.1103/PhysRevLett.100.191601",
      eprint         = "0802.3318",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "SU-ITP-08-02, MIT-CTP-3929",
      SLACcitation   = "%%CITATION = ARXIV:0802.3318;%%"
}

@article{Grozdanov:2015kqa,
      author         = "Grozdanov, Sašo and Kaplis, Nikolaos",
      title          = "{Constructing higher-order hydrodynamics: The third
                        order}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "6",
      pages          = "066012",
      doi            = "10.1103/PhysRevD.93.066012",
      eprint         = "1507.02461",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1507.02461;%%"
}


@article{Grozdanov:2016zjj,
      author         = "Grozdanov, Saso and van der Schee, Wilke",
      title          = "{Coupling constant corrections in holographic heavy ion
                        collisions}",
      year           = "2016",
      eprint         = "1610.08976",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "MIT-CTP-4850",
      SLACcitation   = "%%CITATION = ARXIV:1610.08976;%%"
}

@article{Kapusta:2011gt,
      author         = "Kapusta, Joseph~I. and Muller, Berndt and Stephanov, Mikhail~A.",
      title          = "{Relativistic Theory of Hydrodynamic Fluctuations with
                        Applications to Heavy Ion Collisions}",
      journal        = "Phys. Rev.",
      volume         = "C85",
      year           = "2012",
      pages          = "054906",
      doi            = "10.1103/PhysRevC.85.054906",
      eprint         = "1112.6405",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1112.6405;%%"
}

@article{Chakraborty:2010fr,
      author         = "Chakraborty, Purnendu and Kapusta, Joseph~I.",
      title          = "{Quasi-Particle Theory of Shear and Bulk Viscosities of
                        Hadronic Matter}",
      journal        = "Phys. Rev.",
      volume         = "C83",
      year           = "2011",
      pages          = "014906",
      doi            = "10.1103/PhysRevC.83.014906",
      eprint         = "1006.0257",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1006.0257;%%"
}



@article{Buchel:2003tz,
      author         = "Buchel, Alex and Liu, James T.",
      title          = "{Universality of the shear viscosity in supergravity}",
      journal        = "Phys. Rev. Lett.",
      volume         = "93",
      year           = "2004",
      pages          = "090602",
      doi            = "10.1103/PhysRevLett.93.090602",
      eprint         = "hep-th/0311175",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "NSF-KITP-03-103, MCTP-03-53",
      SLACcitation   = "%%CITATION = HEP-TH/0311175;%%"
}

@article{Fuini:2016qsc,
      author         = "Fuini, John F. and Uhlemann, Christoph F. and Yaffe,
                        Laurence G.",
      title          = "{Damping of hard excitations in strongly coupled $
                        \mathcal{N} = 4$ plasma}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2016",
      pages          = "042",
      doi            = "10.1007/JHEP12(2016)042",
      eprint         = "1610.03491",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1610.03491;%%"
}

@article{Horowitz:1999jd,
      author         = "Horowitz, Gary T. and Hubeny, Veronika E.",
      title          = "{Quasinormal modes of AdS black holes and the approach to
                        thermal equilibrium}",
      journal        = "Phys. Rev.",
      volume         = "D62",
      year           = "2000",
      pages          = "024027",
      doi            = "10.1103/PhysRevD.62.024027",
      eprint         = "hep-th/9909056",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "NSF-ITP-99-70",
      SLACcitation   = "%%CITATION = HEP-TH/9909056;%%"
}

@article{Amado:2007yr,
      author         = "Amado, Irene and Hoyos-Badajoz, Carlos and Landsteiner,
                        Karl and Montero, Sergio",
      title          = "{Residues of correlators in the strongly coupled N=4
                        plasma}",
      journal        = "Phys. Rev.",
      volume         = "D77",
      year           = "2008",
      pages          = "065004",
      doi            = "10.1103/PhysRevD.77.065004",
      eprint         = "0710.4458",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IFT-UAM-CSIC-07-53",
      SLACcitation   = "%%CITATION = ARXIV:0710.4458;%%"
}


@article{Huovinen:2006jp,
      author         = "Huovinen, Pasi and Ruuskanen, Pentti~V.",
      title          = "{Hydrodynamic Models for Heavy Ion Collisions}",
      journal        = "Ann. Rev. Nucl. Part. Sci.",
      volume         = "56",
      year           = "2006",
      pages          = "163-206",
      doi            = "10.1146/annurev.nucl.54.070103.181236",
      eprint         = "nucl-th/0605008",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0605008;%%"
}

@article{Kolb:2003dz,
      author         = "Kolb, Peter F. and Heinz, Ulrich W.",
      title          = "{Hydrodynamic description of ultrarelativistic heavy ion
                        collisions}",
      year           = "2003",
      pages          = "634-714",
      eprint         = "nucl-th/0305084",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "SUNY-NTG-03-06",
      SLACcitation   = "%%CITATION = NUCL-TH/0305084;%%"
}

@book{Misner:1974qy,
      author         = "Misner, Charles W. and Thorne, K. S. and Wheeler, J. A.",
      title          = "{Gravitation}",
      publisher      = "W. H. Freeman",
      address        = "San Francisco",
      year           = "1973",
      journal        = "San Francisco 1973, 1279p",
      ISBN           = "9780716703440, 9780691177793",
      SLACcitation   = "%%CITATION = INSPIRE-95654;%%"
}

@article{Rischke:1998fq,
      author         = "Rischke, Dirk~H.",
      title          = "{Fluid dynamics for relativistic nuclear collisions}",
      booktitle      = "{Hadrons in dense matter and hadrosynthesis. Proceedings,
                        11th Chris Engelbrecht Summer School, Cape Town, South
                        Africa, February 4-13, 1998}",
      journal        = "Lect. Notes Phys.",
      volume         = "516",
      year           = "1999",
      pages          = "21",
      doi            = "10.1007/BFb0107310",
      note           = "[,21(1998)]",
      eprint         = "nucl-th/9809044",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/9809044;%%"
}
